Synthesizing Adversarial Visual Scenarios for Model-Based Robotic Control

Today's robots often interface with data-driven perception and planning models with classical model-predictive controllers (MPC). Often, such learned perception/planning models produce erroneous waypoint predictions on out-of-distribution (OoD) or even adversarial visual inputs, which increase control costs. However, today's methods to train robust perception models are largely task-agnostic - they augment a dataset using random image transformations or adversarial examples targeted at the vision model in isolation. As such, they often introduce pixel perturbations that are ultimately benign for control. In contrast to prior work that synthesizes adversarial examples for single-step vision tasks, our key contribution is to synthesize adversarial scenarios tailored to multi-step, model-based control. To do so, we use differentiable MPC methods to calculate the sensitivity of a model-based controller to errors in state estimation. We show that re-training vision models on these adversarial datasets improves control performance on OoD test scenarios by up to 36.2% compared to standard task-agnostic data augmentation. We demonstrate our method on examples of robotic navigation, manipulation in RoboSuite, and control of an autonomous air vehicle.

==> figures_latex/all_metrcs_table.tex <==
\begin{figure}[h]
\begin{tabular}{|c|c|c|c|c|}\hline
Domain & Network & Dataset & \makecell{Avg MPC Cost} & \makecell{Avg Waypoint Error} \\\hline
Toy  & Original & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
Toy  & Data Aug & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
Toy  & CURL & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
Toy  & Random Sampling & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
Toy  & Task Driven & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\hline
\end{tabular}

\vspace{1cm}
% \begin{tabular}{|c|c|c|c|c|}\hline
% Manipulation  & Original & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
% Manipulation  & Data Aug & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
% Manipulation  & CURL & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
% Manipulation  & Random Sampling & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
% Manipulation  & Task Driven & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
%      &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\hline
% \end{tabular}
% \\
\begin{tabular}{|c|c|c|c|c|}\hline
X-plane  & Original & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
X-plane  & Data Aug & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
X-plane  & CURL & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
X-plane  & Random Sampling & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\midrule
X-plane & Task Driven & $\datasetorigtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetoodtest$ & $33.6 \%$ & $66.1 \%$ \\[3pt]
     &          & $\datasetadvtest$ & $49.9 \%$ & $51.5 \%$ \\\hline
% Manipulation & $\datasetoodtest$ & $29.1 \%$ & $37.1 \%$ \\[3pt]
%                       & $\datasetadvtest$ & $36.2 \%$ & $32.8 \%$ \\\midrule
% X-plane & $\datasetnighttest$ & $36.2 \%$ & $89.2 \%$ \\[3pt]
%                       & $\datasetadvtest$ & $41.7 \%$ & $69.1 \%$ \\[2pt]\hline
\end{tabular}
\caption{A}\label{tab:all_metrics_table}
\end{figure}


==> figures_latex/architecture.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{images/architecture.pdf}
    \caption{\small{ \textbf{Differentiable Robot Learning Architecture:} 
    A robot measures a visual scene $s$, which it maps through an encoder to yield scene embedding $z$. Given a history of waypoints $w_p$, a task module (planner) outputs a future set  of waypoints $w_F$ to track. Finally, these waypoints are tracked using a differentiable model predictive controller (MPC) that outputs a task cost $J$. We assume scenes $s$ are rendered by a generative model, such as a differentiable renderer, that maps latent parameters describing a scene $\nu$ to an image $s$.
    \textbf{Our key contribution} is to train an adversary (orange) to generate synthetic, but realistic, images $\bar{s}$ that are poor for the current planner and controller. These scenes are then used to re-train the planning module for robust performance on OoD data.}}
    \label{fig:expr_arch}
    % \vspace{-1em}
\end{figure*} 

% original
%    \caption{\small{ \textbf{Differentiable Robot Learning Architecture:} A block-diagram representing information flow in a learning-based robotic system. Adversary (orange) and differential renderer (blue) are part of our method. Differential renderer (blue) is trained separately and its kept frozen during adversarial scenario generation procedure (Algorithm \ref{alg:train}). Only the adversary (orange) is trained during adversarial scenario generation (Algorithm \ref{alg:train}).  All the blocks are described in detail in section \ref{sec:proposed_method}.   }}


==> figures_latex/collision_toy_scenario.tex <==
\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.49\textwidth}
    \caption{\small{\textbf{Our method improves collision avoidance on challenging motion planning environments}: We show the number of collisions with an obstacle for different training schemes on the original, OoD, and synthetic adversarial test environments. A single collision occurs when the MPC-enacted trajectory intersects an ellipsoidal obstacle. The columns represent how many scenarios of the 2200 test scenarios had even a single collision for held-out test datasets $\datasetorigtest$, $\datasetoodtest$ and $\datasetadvtest$ respectively. 
    The best performance is bolded and rows correspond to benchmark schemes.}}
    %All the different training schemes are compared in rows on the above mentioned metrics.}}     
    \vspace{2mm}

    \label{tab:toy_collision}
    \centering
    % \captionof{}{2D Obstacle Avoidance Collision Comparisons}
    \begin{tabular}{|c|c|c|c|}
        \hline
        Algorithm & $\datasetorigtest$ & $\datasetoodtest$ & $\datasetadvtest$  \\ \hline
        \hline
        \textsc{Original}  & 389  & 585 & 1058  \\ \hline
        \textsc{Data-Added}  & \textbf{314}  & 552  & 1044 \\ \hline
        \textsc{Data Augment}  & 321 & 489 & 933  \\ \hline
        \textsc{Task-Driven (Ours)}  & 334 & \textbf{422} & \textbf{623} \\ \hline
    \end{tabular}
        \vspace{-0.5em}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.49\textwidth}
        % \includegraphics[width=\columnwidth]{images/ToyScenarioCol.png}
        \includegraphics[width=\columnwidth]{images/ToyScenario_1col.png}
        \caption{\small{\textbf{Our method's Synthesized Adversarial Scenarios:} The robot's goal is to navigate from a start location at $(0, 0)$ to the goal at $(100, 100)$ (green star). Original Scene (Top): The blue obstacles (4 ellipsoids) represent the original scene. Adversarial Scene (Bottom): The red obstacles in the bottom are adversarially created using our method for the original scenario above it. The waypoint trajectories (small sequential dots) are generated by the \texttaskmodel \space for the corresponding scene, and MPC task cost is given in the title. Clearly, the adversarial scenario generates much higher MPC costs by moving the obstacles in the robot's intended path. Crucially, the waypoint trajectory generated by our \textit{re-trained} \textsc{Task Driven} scheme (yellow) learns to better avoid the obstacles with lower MPC cost. Fig. \ref{fig:more_toy_adv} shows additional examples. } }
        \label{fig:toy_adv_scenarios}
    \vspace{-1em}
  \end{minipage}
\end{figure}

==> figures_latex/combined_metrics_curl.tex <==
\begin{figure*}[t]
    % \includegraphics[width=1.0\textwidth]{images/box_metrics.pdf}
    \begin{center}
    \includegraphics[width=1\textwidth]{images/legend_curl.png}
    \includegraphics[width=1\textwidth]{images/all_plots_curl.png}
    \end{center}
    \caption{\edits{\small{\textbf{Benefits of Task-Driven Data Augmentation for Simple 2D Motion Planning, Robot Manipulation and X-Plane Dataset}}}}
     \label{fig:combined_metrics_curl}
\vspace{-1em}
\end{figure*}


==> figures_latex/combined_scenario.tex <==
\begin{figure}[!tbp]
  \begin{minipage}[b]{0.65\textwidth}
    \includegraphics[width=\textwidth]{images/ToyScenario_1col.png}
    \caption{\small{\textbf{Our method's Synthesized Adversarial Scenarios:} The robot's goal is to navigate from a start location at $(0, 0)$ to the goal at $(100, 100)$ (green star). Original Scene (Top): The blue obstacles (4 ellipsoids) represent the original scene. Adversarial Scene (Bottom): The red obstacles in the bottom are adversarially created using our method for the original scenario above it. The waypoint
    trajectories (small sequential dots) are generated by the \texttaskmodel \space for the corresponding scene, and MPC task cost is given in the title. Clearly, the adversarial scenario generates much higher MPC costs by moving the obstacles in the robot's intended path. Crucially, the waypoint trajectory generated by our \textit{re-trained} \textsc{Task Driven} scheme (yellow) learns to better avoid the obstacles with lower MPC cost. Fig. \ref{fig:more_toy_adv} shows additional examples. } }
    \label{fig:toy_adv_scenarios}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.34\textwidth}
    \includegraphics[width=\textwidth]{images/Robosuite.png}
    \caption{\small{\textbf{Our method's Synthesized Adversarial Scenarios:} The robot's goal is to navigate from a start location at $(0, 0)$ to the goal at $(100, 100)$ (green star). Original Scene (Top): The blue obstacles (4 ellipsoids) represent the original scene. Adversarial Scene (Bottom): The red obstacles in the bottom are adversarially created using our method for the original scenario above it. The waypoint
    trajectories (small sequential dots) are generated by the \texttaskmodel \space for the corresponding scene, and MPC task cost is given in the title. Clearly, the adversarial scenario generates much higher MPC costs by moving the obstacles in the robot's intended path. Crucially, the waypoint trajectory generated by our \textit{re-trained} \textsc{Task Driven} scheme (yellow) learns to better avoid the obstacles with lower MPC cost. Fig. \ref{fig:more_toy_adv} shows additional examples. } }
    \label{fig:manipulation_adv_scenarios}
  \end{minipage}
 \vspace{-1em}
\end{figure}

==> figures_latex/combined_xplane_adv_tsne.tex <==
\begin{figure}[!tbp]
 \begin{minipage}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/xplane_adv_scenario_single.pdf}
    \caption{\small{\textbf{X-Plane Synthetic Adversarial Scenarios:} 
    %This figure shows two scenarios created by our adversarial training.  
    The top row contains images from the original dataset with the corresponding ground-truth label waypoint (distance to center-line and heading angle), as well as MPC task cost if this waypoint was correctly followed. The bottom row shows the corresponding adversarial scenario generated by our method. As expected, both the adversarial scenarios lead to higher MPC costs. On the left, the adversary learns to blur the runway center-line to emulate a foggy condition, while the
    right image emulates an OoD night scenario where only the center-line (top left) is faintly visible. Fig. \ref{fig:more_toy_adv} shows additional examples.}}
    \label{fig:adv_scenarios}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/xplane_latent.png}
    \caption{\small{\textbf{X-Plane VAE Latent Space Visualization:} We reduce the dimension of X-Plane test datasets to visualize their relative distance using the t-SNE method \cite{hinton2002stoc}. Recall that the perception module $z = \mpercep (s; \percepparam)$  takes an image $s$ of the scene as input and outputs a latent representation $z$ of the scene. Each dataset contains scenes $s$, and we visualize the corresponding latent variables $z$ after passing the scenes through the perception module. The key takeaway is that the \textit{Task Driven} scenes are very close to the OoD \textit{Night} scenes, which explains why our \TaskDriven \space model performs so well on the OoD \textit{Night} dataset. Additionally, the \textit{Data Augmentation} scenes are not at all close to \textit{Night} scenes, thus explaining why the \DataAug \space task model is not able to generalize to  the OoD \textit{Night} dataset. This visualization demonstrates how our task-driven method targetedly generates synthetic
    scenarios to aid generalization on OoD data.}} 
    \label{fig:xplane_latent}
  \end{minipage}
 \vspace{-1em}
\end{figure}

==> figures_latex/toy_adv_scenrio.tex <==
% \begin{figure}[t]

% \subfloat[]{%
%   \includegraphics[clip,width=\columnwidth]{images/toy_2adv_scenario.pdf}%
%   \label{fig:adv_scenarios1}
% }

% % \subfloat[]{%
% %   \includegraphics[clip,width=\columnwidth]{images/adv_recon_10.png}%
% %   \label{fig:adv_scenarios1}
% % }



% \end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/toy_2adv_retrained.png}
    \caption{\small{\textbf{Our method's Synthesized Adversarial Scenarios:} The robot's goal is to navigate from a start location at $(0, 0)$ to the goal at $(100, 100)$ (green star). \textbf{Original Scenes (Top Row):} The blue obstacles (4 large ellipsoids) represent two distinct original scenes. \textbf{Corresponding Adversarial Scenes (Bottom Row:) } The red obstacles in the bottom row are adversarially created using our method for the corresponding original scenario above it. The waypoint
    trajectories (small sequential dots) are generated by the \texttaskmodel \space for the corresponding scene, and MPC task cost is given in the title. Clearly, the adversarial scenarios (bottom row) generate significantly higher MPC costs by moving the obstacles in the robot's intended path. Crucially, the waypoint trajectory generated by our \textit{re-trained} \textsc{Task Driven} scheme (yellow) learns to better avoid the obstacles and thus achieves a lower MPC Cost. } }
    \label{fig:toy_adv_scenarios}
\vspace{-1em}
\end{figure*}

%\caption{\small{\textbf{Toy Synthetic Adversarial Scenarios:} This figure shows two toy scenarios created by the adversarial training. Robot's goal is to navigate from Start $(0, 0)$ to the goal $(100, 100)$ (green star). The blue obstacles (large four ellipsoids) in the top row represent two distinct original scenes. The red obstacles (large four ellipsoids) in the bottom row are adversarially created using our method for the corresponding original scenario above it. The waypoint trajectories (small sequential dots) are generated by the \texttaskmodel \space for the corresponding scene. The corresponding MPC cost (the \texttaskcost) is shown as the title of each figure. The adversarial scenarios (bottom row) generate significantly higher MPC costs by moving the obstacles in the robot's path. Finally, the waypoint trajectory generated by our \textsc{Task Driven} is shown in yellow. Our \texttaskmodel, \textsc{Task Driven}, better learns to avoid the adversarial obstacles and thus achieve a lower MPC Cost. } }



==> figures_latex/toy_cost_box_plots.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/toy_cost.png}
    \caption{
    \small{ \textbf{Toy Example MPC Cost Comparisons:} This figure shows the MPC cost or \texttaskcost \taskcost for Task Models \textsc{Original} (blue), \textsc{Data Added} and \textsc{Task Driven} (red) on 2200 test data scenarios. The X-axis shows the different test datasets \textit{Original} $\datasetorigtest$ and \textit{Synthetic Adversarial} $\datasetadvtest$. The Y-axis has the normalized MPC costs (lower being better). Our \texttaskmodel  \textsc{Task Driven} (red) works on par with other \texttaskmodels on the  \textit{Original} test data, however it significantly outperforms (smaller MPC Costs) other \texttaskmodels on the challenging scenarios in the \textit{Synthetic Adversarial} test dataset. }}
     \label{fig:toy_box_plots}
\vspace{-1em}
\end{figure}


==> figures_latex/toy_metrics.tex <==
\begin{figure*}[t] \label{fig:toy_box_plots}
\subfloat {
    \includegraphics[width=0.5\textwidth]{images/new_toy_cost.png} % first figure itself
    \label{fig:toy_mpc_orig}
    }
\subfloat
{
    \includegraphics[width=0.5\textwidth]{images/new_toy_wpt.png} % first figure itself
    \label{fig:toy_mpc_adv}
}
% {
%     \includegraphics[width=0.3\textwidth]{wpt_err_box_plot_1k 2.png} % first figure itself
%     \label{fig:toy_wpt}
% }

    \caption{\small{\textbf{Benefits of Task-Driven Data Augmentation for Simple Motion Planning :} We show the MPC task cost $J$ (left) and MSE for waypoint predictions for the \textsc{Original} (blue), \textsc{Data Added} (yellow), \DataAug \space (green) and \textsc{Task Driven} (red) schemes on 2200 held-out test environments. The x-axis shows different test conditions, and lower \texttaskcost \space and waypoint MSE (y-axis) are better. Our \textsc{Task Driven} scheme (red) works on par with other
    \texttaskmodels \space on the \textit{Original} test data for both metrics. However, it significantly outperforms other \texttaskmodels \space on challenging scenarios in the \textit{out-of-distribution (OoD)} dataset, and \textit{Synthetic Adversarial} test datasets. Crucially, our \textsc{Task Driven} scheme (red) is able to generalize much better to \textit{OoD} dataset compared all other training schemes. The \textsc{Data Added} training scheme has high variance on \textit{OoD} and \textit{Synthetic Adversarial} datasets since it overfits to the \textit{Original} dataset. }} 
    %Additionally, is noteworthy that \textsc{Original} (blue) and \textsc{Data Added} (yellow) schemes perform poorly on the \textit{Synthetic Adversarial} test dataset, confirming that our method indeed synthesizes adversarial environments.}}
\vspace{-1em}
\end{figure*}


% SOMI OLD: 
%\caption{\small{\textbf{Toy Example Task Model Comparisons:} The figure shows the \texttaskcost \taskcost (left) and the mean-squared Waypoint Error (right) for the Task Models \textsc{Original} (blue), \textsc{Data Added} (yellow) and \textsc{Task Driven} (red) on 2200 test data scenarios. The X-axis shows the different test datasets \textit{Original} $\datasetorigtest$ and \textit{Synthetic Adversarial} $\datasetadvtest$. Lower \texttaskcost \space and lower waypoint MSE are better. Our \texttaskmodel \space \textsc{Task Driven} (red) works on par with other \texttaskmodels \space on the  \textit{Original} test data for both metrics, and it significantly outperforms other \texttaskmodels \space on the challenging scenarios in the \textit{Synthetic Adversarial} test dataset. Additionally, it is important to note that both Task Models \textsc{Original} (blue) and \textsc{Data Added} (yellow) perform poorly on the  \textit{Synthetic Adversarial} test dataset, thus showing that the scenarios created by our method are indeed adversarial. }}



==> figures_latex/toy_scenario.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{images/toy_scenario.pdf}
    \caption{\small{\textbf{Toy scenarios}:
    A scenario for the toy task is demonstrated. Robot's goal is to navigate from Start $(0, 0)$ to the goal $(100, 100)$ (green star). Ellipsoid obstacles are shown in blue. Robots current location is shown as a yellow dot. Green waypoints, representing history $\mathbf{w}_P$ and the scene $s$ (only obstacles and goal) is given as input to the  \texttaskmodel $\mtaskmodel$, which outputs blue waypoints $\mathbf{w}_F$. Red waypoints show the ground truth trajectory. Yellow line is the trajectory generated by the MPC. }} \label{fig:toy_scenario}
\vspace{-1em}
\end{figure}


==> figures_latex/toy_wpy_err.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/toy_wpt.png}
    \caption{\small{
    \textbf{Toy Example Waypoint Error Comparisons:} This figure shows the mean squared waypoint error between cost or \texttaskcost \space $\taskcost$ for Task Models \textsc{Original} (blue), \textsc{Data Added} and \textsc{Task Driven} (red) on 2200 test data scenarios. The X-axis shows the different test datasets \textit{Original} $\datasetorigtest$ and \textit{Synthetic Adversarial} $\datasetadvtest$. The Y-axis has the normalized MPC costs (lower being better). Our \texttaskmodel \space \textsc{Task Driven} (red) works on par with other \texttaskmodels \space on the  \textit{Original} test data, however it significantly outperforms (smaller MPC Costs) other \texttaskmodels \space on the challenging scenarios in the \textit{Synthetic Adversarial} test dataset.
    
    This figure shows the mean squared waypoint error between Task Model's prediction and ground truth. Left box plots were evaluated on test dataset $\xi$ and right box plots were evaluated on test adversarial dataset $\bar{\xi}$. Y-axis has the MSE waypoint error for Task Models \emph{Original}, \emph{Data Added} and \emph{Task Driven}. 
    }}
    \label{fig:toy_wpt}
\vspace{-1em}
\end{figure}


==> figures_latex/xplane_metric.tex <==
\begin{figure*}[ht!] \label{fig:xplane_mpc}
\subfloat {
    \includegraphics[width=0.5\textwidth]{images/xplane_mpc.png}
    \label{fig:toy_mpc_orig}
    }
\subfloat
{
    \includegraphics[width=0.5\textwidth]{images/xplane_wpt.png}
    \label{fig:toy_mpc_adv}
}
\caption{\small{\textbf{Task-Driven Data Augmentation Improves Control Performance on the X-Plane Dataset:}
    We show improvements for the MPC task cost $\taskcost$ (left) and waypoint prediction error (right) for our \textsc{Task Driven} method (red) compared to benchmarks on 11,000 challenging test data scenarios. The x-axis shows the diverse held-out test dataset scenarios. Our \textsc{Task Driven} scheme (red) works on par with other \texttaskmodels \space on the  \textit{Original} (afternoon) and similar \textit{Morning} test datasets. Crucially, it significantly outperforms other schemes on
    naturally-occurring OoD \textit{Night} scenarios and \textit{Synthetic Adversarial} test datasets. Importantly, we beat today's method of task-agnostic data augmentation (green) which often applies image augmentations that are ultimately benign for the model-based controller.}}
\vspace{-1em}
\end{figure*}


%The figure shows the \texttaskcost, $\taskcost$, (left) and the mean-squared Waypoint Error (right) for the Task Models \textsc{Original} (blue), \textsc{Data Added} (yellow), \textsc{Data Augmentation} (green) and \textsc{Task Driven} (red) on 11000 test data scenarios. The X-axis shows the different test datasets \textit{Original} $\datasetorigtest$, \textit{Morning} $\datasetmorningtest$, \textit{Night} $\datasetnighttest$, and \textit{Synthetic Adversarial} $\datasetadvtest$. Lower \texttaskcost \space and lower waypoint MSE are better. Our \texttaskmodel \space \textsc{Task Driven} (red) works on par with other \texttaskmodels \space on the  \textit{Original} and \textit{Morning} test datasets, and it significantly outperforms other \texttaskmodels \space on the challenging scenarios in the  \textit{Night} and \textit{Synthetic Adversarial} test datasets. Additionally, it is important to note that both Task Models \textsc{Original} (blue) and \textsc{Data Added} (yellow) perform poorly on the  \textit{Synthetic Adversarial} test dataset, thus showing that the scenarios created by our method are indeed adversarial. }}



==> figures_latex/xplane_mpc.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/xplane_mpc.png}
    \caption{\small{ Figure shows the \texttaskcost $\taskcost$ on different test data scenarios for different training scheme (separated by color of box plot). Y-axis has the waypoint MSE (lower being better).}}
    \label{fig:xplane_mpc}
\vspace{-1em}
\end{figure}


==> figures_latex/xplane_wpt.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/xplane_wpt.png}
    \caption{\small{
     Figure shows the waypoint MSE between Task Model's prediction and ground truth on different test data scenarios. Y-axis has the waypoint MSE (lower being better). Box plots represent the corresponding training scheme.
    }}
    \label{fig:xplane_wpt}
\vspace{-1em}
\end{figure}

==> sections/abstract.tex <==
A variety of robots are increasingly using data-driven perception and planning models
that interface with classical model-based controllers. For example, drones can use computer vision models
to estimate target landing sites or navigation waypoints, which can be tracked by model predictive control (MPC). 
Often, such learned perception and planning models can be harmed by adversarial examples, which produce
erroneous state estimates or waypoints that ultimately lead to increased control costs. 
In contrast to prior work that synthesizes adversarial examples for single-step vision tasks, the key novelty of our work is to efficiently synthesize adversarial scenarios for multi-step, model-based control tasks. To do so, we leverage recently-developed differentiable MPC methods to calculate the sensitivity of a model-based controller to errors in state estimation, which in turn guides how we learn to synthesize adversarial visual scenarios. We illustrate that fine-tuning learned vision and
planning models on these adversarial datasets improves robustness on unseen test scenarios by up-to \SC{28.2\%} compared to standard task-agnostic data augmentation. 
Our system is tested on a robotic navigation example and on a photo-realistic autonomous aircraft simulation engine. 

%A variety of robots are increasingly using data-driven perception and planning models
%that interface with classical model-based controllers. For example, drones can use computer vision models
%to estimate target landing sites or navigation waypoints, which can be tracked by model predictive control (MPC). 
%Often, such learned perception and planning models can be harmed by adversarial examples, which produce
%erroneous state estimates or waypoints that lead to increased costs for an ultimate control task. 
%In this paper, we present a method to automatically synthesize adversarial visual scenarios
%for model-based control tasks. In contrast to prior work that synthesizes adversarial examples
%for single-step vision tasks, we calculate the sensitivity of a model-based controller to errors in state
%estimation, which guides efficient design of adversarial scenarios. We illustrate that fine-tuning
%learned vision and planning models on these adversarial datasets improves robustness on unseen test scenarios
%by up-to $X \times$, including on a photo-realistic autonomous aircraft simulator.


==> sections/checklist.tex <==
% For the paper checklist
\newcommand{\answerYes}[1]{{\color{blue}{[Yes]#1}}}
\newcommand{\answerNo}[1]{{\color{red}{[No]#1}}}
\newcommand{\answerNA}[1]{{\color{red}{[N/A]#1}}}
\newcommand{\answerTODO}[1]{{\color{red}{\bf[TODO]}}}

\noindent \textbf{Paper Submission Checklist}

\noindent \textbf{Student Name: Shubhankar Agarwal} \newline
\noindent \textbf{Peer Reviewer Name: Po-Han}  \newline
\noindent \textbf{Paper Title: Towards  Robust  Vision-Based  Robotic  Control  using  Adversarial Scenario  Generation} \newline
\noindent \textbf{Date: 01/04/2022} \newline

\begin{enumerate}
    \item Did you spell check and grammar check the full document, using Grammarly if needed?
    \answerYes{}
    \item Did you organize the LaTeX files according to the sample paper guide, including naming the file appropriately, organizing sections etc.? \answerYes{}
  \item Did you make sure all plots are legible, in at least 20 point font, and ideally use the lab plotting tools/guidelines? \answerYes{}
  \item Did you have another student in the lab peer review your paper for clarity, typos, wrong notation etc.? Send an email to Sandeep (CC'ing both students) with the paper draft. \answerYes{}
  \item Did you make sure all references have the book/conference venue, not just the author and title? \answerNo{}
  \item Did you use the common reference files in the lab GIT, making sure to put our internal papers in ref/SwarmLabPubs.bib and all other papers in ref/external.bib? \answerNo{}
  \item Did you outline your paper and place the DARPA Heilmeier Catechism question answers at the top of the outline? \answerYes{}
\end{enumerate}


\newpage


==> sections/conclusions.tex <==
This paper presents a principled method to automatically synthesize adversarial scenarios
for vision-based robotic control. Our first key insight is that today's adversarial example generation
is largely limited to single-step inference and computer vision tasks, not multi-step planning tasks.
As such, our key contribution is to compute the sensitivity of model-based control tasks to perception errors, which in turn
guides how an adversary learns to generate hard-to-control visual examples. Moreover, by re-training on these synthesized adversarial examples, our method is able to generalize better to new test datasets than today's task-agnostic data augmentation schemes. Our experiments on toy synthetic navigation problems and the photo-realistic X-Plane simulator demonstrate our approach can out-perform task-agnostic data augmentation by up to $28.2\%$ on the out-of-distribution scenarios.

In future work, we plan to provide theoretical guarantees for an illustrative example with a linear adversary, simple linear renderer/scene generator, and linear MPC control problem. Moreover, we plan to compare how adversarial examples for single-step vision tasks differ from those generated by our synthesis approach for multi-step control problems. Finally, we plan to test the generalization ability of our approach on a small mobile robot operating in OoD lighting, weather, and terrain
conditions. 
%compared to its training distribution.


==> sections/experiments.tex <==

We now evaluate \SC{our method (Algorithm \ref{alg:train})} on two diverse tasks. 
\SC{The first task is a simple, but illustrative, toy example of robotic motion planning.}

First, we start with a simple synthetically created toy example to benchmark our proposed method. The second experiment is a more practical task where an airplane is trying to taxi at an airport based on the vision input in different weather conditions simulated in a photo-realistic simulator.

\subsection{Experiment Preliminaries} \label{sec:expr_prelim}

\textit{Adversary Model:} We use a linear model for our adversary $\adv( \nu ; \advparam ) $. That is for a given 
$\nu \in \mathbb{R}^{n} $, we will have $ \adv( \nu ; \advparam ) =  \advparam \nu $ and $\advparam \in \mathbb{R}^{n \times n }$. We decided to use a linear adversary to make analytical gradient computation for training. Rest of the gradients will be calculated using automatic differentiation libraries.
Nonlinear and more complex adversarial models can also be used, but it is not relevant for our method.

% Gradient of a linear adversary w.r.t to its parameters $\advparam$ will simply be $\frac{\partial f}{\partial \advparam } = \frac{\partial \advparam \nu}{\partial \advparam }  = {\nu}^{\top} $.
    
    % Gradient calculation of Task Cost $\hat{J}(  \theta, \advparam )$ in equation \ref{eq:adv_grad} with a linear adversary are shown in equations \ref{eq:expr_grad}.
    % \begin{subequations} \label{eq:expr_grad}
    %     \begin{align} 
    %     % \frac{\partial \hat{J}(  \theta, \advparam )}{\partial \advparam} &= \frac{\partial \hat{J}(  \theta, \advparam )}{\partial \theta} \cdot \frac{\partial \theta}{\partial f } \cdot \frac{\partial f}{\partial \advparam } \\
    %     \frac{\partial f}{\partial \advparam } &= \frac{\partial \advparam^T \theta}{\partial \advparam }  = {\theta}^{\top} 
    % \end{align}
    % \end{subequations}
    % $\frac{\partial \hat{J}(  \theta, \advparam )}{\partial \theta}$ and $\frac{\partial \theta}{\partial f } $ will be calculated using automatic differentiation libraries. 
    
\textit{Distance Loss and Regularization:} We will use the Mean-Squared Error as the distance loss $\distloss$ in \eqref{eq:adv_loss}. That is $\distloss = \left|\left| \nu - \bar{\nu} \right|\right|_{2} ^{2} $. Gradient of distance loss w.r.t to adversary parameters $\advparam$ is shown in eq. \ref{eq:dist_loss_grad}.
    
    \begin{equation} \label{eq:dist_loss_grad}
        \begin{aligned} 
        \frac{\partial \distloss }{\partial \advparam } = -2 \cdot \frac{\partial \bar{\nu} }{\partial \advparam } \cdot {\nu}^{\top}  (\nu - \bar{\nu} )
    \end{aligned}
    \end{equation}
    $\frac{\partial \bar{\nu} }{\partial \advparam } $ will be calculated using automatic differentiation libraries. $\kappa$ is set manually based on the task.

    % We will use $q=2$-norm (ridge regularizer) for the regularized term $||\advparam||_{q} = \left|\left| \advparam \right|\right|_{2} ^{2}$ in equation \ref{eq:adv_loss}. Gradient calculations for regularizer loss are trivial. $\kappa$ and $\lambda$ are set manually based on the task.
    
    % \item We will use $p=2$-norm (ridge regression) for the regularized term $||\advparam||_{p} = \left|\left| \advparam \right|\right|_{2} ^{2}$ in equation \ref{eq:adv_loss}. $\kappa$ and $\lambda$ are set manually based on the task.
    
    % \begin{subequations} \label{eq:regur_loss_grad}
    %     \begin{align} 
    %     \mathcal{I}(x, \bar{x}) &= \left|\left| x - \bar{x} \right|\right|_{2} ^{2} \\
    %     \frac{\partial \mathcal{I}(x, \bar{x})}{\partial \advparam } &= -2 \cdot \frac{\partial \bar{x} }{\partial f } \cdot \frac{\partial f}{\partial \advparam } (x - \bar{x} ) \\
    %     \frac{\partial \mathcal{I}(x, \bar{x})}{\partial \advparam } &= -2 \cdot \frac{\partial \bar{x} }{\partial f } \cdot {\theta}^{\top}  (x - \bar{x} ) \\
    % \end{align}
    % \end{subequations}

\textit{Variational Autoencoder (VAE):} We will use a VAE as the differentiable rendering module $ \render$ (defined in section \ref{sec:diff_rendr_module}). The VAEs have gained significant popularity recently because of their multi-modal data generation capabilities and stabler training (compared to Generative Adversarial Networks (GANs)). Additionally, the VAEs encode data input $x$ in a lower-dimensional subspace (the latent space) from the original higher-dimensional space. It is important to note that we only use the VAE \textit{Decoder} as the differentiable rendering module, which takes parameters $\nu$ as input and outputs the image $s$ of the scene. We keep the \textit{Decoder} frozen after training it initially on the whole dataset.

% We will use Variational Autoencoder (VAE) (CITE) as the differentiable rendering module $ \psi(\theta)$ (defined in section \ref{sec:diff_rendr_module}).  VAE for the both the tasks were trained using ELBO loss. Encoder and Decoder are each have 3 convolutions layers, with ReLU as activation function. Both experiments have different latent dimension size, $|z| = 16$ for experiment \ref{sec:toy_obs} and $|z| = 128$ for experiment \ref{sec:toy_obs}.


\textit{Model Predictive Control (MPC):} In both the tasks, we will formulate the \texttaskcost \space $\taskcost(\mathbf{w}_F)$ as a MPC problem, with quadratic costs and linear constraints. The MPC formulation, shown in \eqref{eq:track_mpc}, receives waypoint vector  $\mathbf{w}_F$ of length F as input to track. $\mpcstate_t \in \mathbb{R}^{4 \times 1}$ is the robot's state at time $t$, defined as $\mpcstate_t = \{l_x, l_y, v, \theta \}$, where $l_x$ and $l_y$ are the robot's $x,y$ location in meters, $v$ is the speed in meters/sec and $\theta$ is robot's angle in radians. $\mpccontrol_t \in \mathbb{R}^{2 \times 1}$ is the robot's control input at time $t$, defined as $\mpccontrol_t = \{a, \gamma \}$, where $a$ is robot's acceleration in $m/s^2$ and $\gamma$ is robot's steering input in radians/sec. $\mathbf{Q} \in \mathbb{R}^{4 \times 4} $ is the state cost matrix and $\mathbf{R} \in \mathbb{R}^{2 \times 2} $ is control cost matrix. $\mathbf{A} \in \mathbb{R}^{4 \times 4} $ and $\mathbf{B} \in \mathbb{R}^{4 \times 2} $ define the robot's dynamics. $u_{min} \leq \mpccontrol_t \leq u_{max}$ define the control constraints, max/min accel and max/min steering angle. $ x_{min} \leq \mpcstate_t \leq x_{max}$ define the state constraints, min/max speed and the linear obstacle avoidance constraints. The linear obstacle avoidance constraints, (only used in toy example) were calculated by drawing perpendicular hyperplanes w.r.t the obstacles. We used the double integral dynamics for the first experiment and the linearized unicycle dynamics for the second experiment.
Given a set of $F$ future waypoints $w_F = \{w_0, w_1, \ldots, w_{F-1}\}$ for a planning horizon starting at $t=0$, our MPC task cost and problem become:  
    \begin{equation} \label{eq:track_mpc}
        \begin{aligned}
            \min_{\mpcstate_{0:F}, u_{0:F-1}} ~\hat{J}(w)  &=\sum_{t=0}^{F} (w_{t}^{\top} - \mpcstate_t^{\top} ) \mathbf{Q} (w_{t} -\mpcstate_t) +\sum_{t=0}^{F-1} \mpccontrol_t^{\top} \mathbf{R} \mpccontrol_t \\
    \text {such that~} & \mpcstate_{t+1} =\mathbf{A}\mpcstate_t + \mathbf{B} \mpccontrol_t \\
    & u_{min} \leq \mpccontrol_t \leq u_{max}  \\
    & x_{min} \leq \mpcstate_t \leq x_{max}.  \\
        \end{aligned}
    \end{equation}
    
We used he \emph{cvxpylayers} \cite{cvxpylayers2019} for backpropagation of the \texttaskcost \space through the \texttaskmodel \space and calculating $\frac{\partial \hat{J}(  \nu, \advparam )}{\partial \nu}$. \emph{Cvxpylayers} is a Python library for constructing differentiable convex optimization layers in PyTorch using CVXPY.

% \SA{CAN BE REMOVED. A convex optimization layer solves a parametrized convex optimization problem in the forward pass to produce a solution and computes the derivative of the solution with respect to the parameters in the backward pass}.
    
\textit{Architectures:} In both the tasks, we used deep networks for the \texttaskmodel \space and the differentiable rendering module $\render$, shown in figure \ref{fig:expr_arch}. The perception module $\mpercep$, is a VAE \textit{Encoder}. Since we are working with images, we used Convolutional Neural Networks (CNNs) for the differentiable rendering module $\render$. We experimented with both MLPs and CNNs for the \texttaskmodel. The type of deep network in the \texttaskmodel \space is not essential for our experiment since our method tries to improve any general \texttaskmodel.

% \input{figures_latex/toy_cost_box_plots}
\input{figures_latex/toy_metrics}


\subsection{Data Schemes} \label{sec:data_schemes}
% We represent a dataset by a tuple of input $x$ and ground-truth label $y$ denoted by $\datasetall$, where $N$ is the number of tuples in the dataset. Specifically, each example $x = (s, \mathbf{w}_P)$ represents robot's image scene input $s$ and the history of waypoints $\mathbf{w}_P$. Using the inputs $x$, the \texttaskmodel \space predicts a ground-truth target vector $y = (\mathbf{w}_F)$ which represents the future waypoints for the robot to follow. 
The subscript in the notation $\dataset$ will represent the type of dataset and the superscript will represent if the dataset is \textit{train} or \textit{test}. 

% We compared the \texttaskmodels \space trained on different datasets as described below. 

We denote the original \textit{train} and \textit{test} dataset by $\datasetorigtrain$ and $\datasetorigtest$. We created another dataset $\datasetaddtrain$ by appending similar data as original dataset to $\datasetorigtrain$. Additionally, we created datasets $\datasetaugtrain$ and $\datasetaugtest$ by performing different image augmentations to the image inputs $s$ in the original datasets $\datasetorigtrain$ and $\datasetorigtest$ respectively. Specifically, we applied random contrast, random brightness and random blur to the images $s$. Augmented datasets contain both the original and augmented data.

Lastly, we created adversarial datasets $\datasetadvtrain$ and $\datasetadvtest$ \space using our method. In order to create the adversarial datasets, we first trained a VAE on $\datasetorigtrain$ to obtain a differentiable rendering module $\render$ and froze the \textit{decoder} weights in the VAE. Next we trained the \texttaskmodel \space $\alltaskmodel$ on the original dataset $\datasetorigtrain$. Finally, we used our method (Algorithm  \ref{alg:train}) to create datasets $\datasetadvtrain$ and $\datasetadvtest$ (from $\datasetorigtest$). Adversarial datasets contain both the original and adversarial data.


% \input{figures_latex/toy_scenario}

\subsection{Illustrative Toy Example: 2D Obstacle Avoidance.} 
\label{sec:toy_obs}
We now introduce a simple task  where a planar 2-D robot has to navigate around obstacles to reach a goal location, as pictured in Figure \ref{fig:toy_adv_scenarios}. This experiment demonstrates how adversarial training creates more challenging scenarios for the \texttaskmodel \space to plan in. Furthermore, after training on the synthetic adversarial scenarios, the \texttaskmodel \space performs much more robustly on synthetic adversarial $\datasetadvtest$

% and original $\datasetorigtest$ datasets.

% Additionally, we quantitatively show that a \texttaskmodel \space trained on adversarial scenarios $\datasetadvtrain$ learns to avoid collisions more successfully and with lower control cost compare to the \texttaskmodel \space trained on $\datasetorigtrain$ and $\datasetaddtrain$.

\textit{Experimental Settings: }

The input to the 2-D planar robot is a $100\times100$ grey-scale image $s$ of the scene, including obstacles and the goal $g$, indicated by a star-shaped marker. Given the sensory input $s$, the \texttaskmodel \space $\alltaskmodel$ is a perception-planning module that outputs a sequence of future waypoints $\mathbf{w}_F$ for the robot to navigate. The \texttaskmodel \space $\mtaskmodel$ uses a history of past waypoints $\mathbf{w}_P$ to improve its predictions. The \texttaskcost \space is a standard quadratic tracking cost with linear obstacle avoidance constraints defined in Equation \ref{eq:track_mpc}.

We synthetically created the training $\datasetorigtrain$ and the held-out test datasets $\datasetorigtest$ for the experiments. The ground truth waypoints $y = \mathbf{w}_F$ are generated using a standard Frenet Planner that has full access to all obstacles and start/goal locations for the entire scene. The synthetic dataset contained $|\datasetorigtrain| = 7000$ training scenarios and $|\datasetorigtest| = 2200$ test scenarios. Larger similar dataset, had $|\datasetaddtrain| = 10000$ training examples. The synthetic adversarial dataset generated by our method had $|\datasetadvtrain| = 10000$ training scenarios (3000 generated adversarially, rest original) and $|\datasetadvtest| = 2200$ test scenarios (all adversarial). We use a history of $P=10$ past waypoints to predict the next $F=20$ future waypoints.

The experiment shows that training the \texttaskmodel \space with additional adversarial data is better for performance than training with additional similar data. We will refer to the \texttaskmodel \space trained on $\datasetorigtrain$ as \textsc{Original}, \texttaskmodel \space trained on $\datasetaddtrain$ as \textsc{Data Added} and \texttaskmodel \space trained on $\datasetadvtrain$ as \textsc{Task Driven}. We quantitatively compare the performance of the above mentioned \texttaskmodels \space on the number of collisions with obstacles, the average \texttaskcost \space $\taskcost$, and the mean-squared error (MSE) in predicting the waypoints. We test these metrics on test dataset $\datasetorigtest$ \space and $\datasetadvtest$. Finally, we qualitatively show that our experiments are adversarial and realistic.

% The experiment shows that a \texttaskmodel \mtaskmodel trained with dataset $\datasetaddtrain$ will have worse performance on the test data $\datasetorigtest$ than a \texttaskmodel \mtaskmodel trained with dataset $\datasetadvtrain$. That is, training the \texttaskmodel \space with additional adversarial data is better for performance than training with a dataset which is similar to the original dataset. We will refer to the \texttaskmodel trained on $\datasetorigtrain$ as \textsc{Original}, \texttaskmodel trained on $\datasetaddtrain$ as \textsc{Data Added} and \texttaskmodel trained on $\datasetadvtrain$ as \textsc{Task Driven}.


% \input{figures_latex/toy_cost_box_plots}
% \input{figures_latex/toy_wpy_err}
\input{figures_latex/collision_table}


\textit{Quantitative results: }
The table \ref{tab:toy_collision} shows the number of collisions in the above-mentioned training schemes. Our \textsc{Task-Driven} approach was able to perform as well as the \textsc{Data-Added} and \textsc{Original} benchmarks on the original test dataset. Additionally, it significantly outperformed the \textsc{Data-Added} scheme by $41\%$ and \textsc{Original} scheme by $48.2\%$ on the adversarial test dataset $\datasetadvtest$. Thus showing our training scheme \textsc{Task-Driven} leads to significantly fewer collisions on challenging out-of-distribution scenarios.

% We now quantify whether our scheme also reduces the task cost (MPC cost $\hat{J}$). 

Figure \ref{fig:toy_box_plots} (left) shows the task cost (MPC) for all training schemes on 2200 held-out \textit{test} data scenarios. On the original test dataset, our \textsc{Task-Driven} scheme (red) performs on par with the \textsc{Original} (blue) scheme and slightly worse than the \textsc{Data-Added} (orange) scheme. \textsc{Data-Added} scheme's performance is natural and expected because it is trained on more original data than the \textsc{Task-Driven} scheme, which allows it to perform slightly better on the original test dataset. However, the key benefits of our approach are shown on the synthetic adversarial test dataset $\datasetadvtest$. The key take-away is that our scheme of \textsc{Task-Driven} has $57.7 \%$ less average cost than \textsc{Data-Added} (Wilcoxon p-value of $0.0$) and $62.9 \%$ compared to \textsc{Original} (Wilcoxon p-value of $0.0$) on the adversarial test dataset.

We now illustrate why our method is able to reduce the ultimate task cost. Specifically, Figure \ref{fig:toy_box_plots} (right) shows that our scheme \textsc{Task-Driven} achieves lower MSE while predicting ground-truth waypoints from the Frenet Planner than competing benchmarks. While all methods perform similarly on the original test dataset $\datasetorigtest$, the key gains of our scheme are on the adversarial test dataset $\datasetadvtest$. Specifically, our scheme of \textsc{Task-Driven} has $78.4 \%$ less average waypoint MSE than \textsc{Data-Added} (Wilcoxon p-value of $0.0$) and $79.3 \%$ compared to \textsc{Original} (Wilcoxon p-value of $0.0$) on the adversarial test dataset.

\textit{Qualitative Results: }
Figure \ref{fig:toy_adv_scenarios} shows some challenging adversarial scenarios that are automatically synthesized by our method in dataset $\datasetadvtrain$. In the two scenarios, our adversarial training scheme brings obstacles closer to the robot's originally intended waypoints and path, making it harder to find a collision-free path. Naturally, this increases the \texttaskcost \space since the robot has to make wider turns with more swerves. Therefore, rather than augmenting our dataset with well-understood scenarios already reflected in the training distribution, our scheme targetedly adds challenging scenarios that makes the model more robust.

% \input{figures_latex/toy_adv_scenrio}
\input{figures_latex/toy_scenario_col}


\subsection{Xplane: Airplane Taxiing} \label{sec:xplane_epr}
\SC{We now} test our method on an autonomous aircraft taxiing problem. The airplane must navigate to the center of \SC{a} runway with minimal control cost 
using visual inputs from a wing-mounted camera in the photo-realistic X-Plane simulator. We use a public dataset from X-Plane consisting of images from the plane's wing-mounted camera in diverse weather conditions and at various orientations relative to the run-way. This standard benchmark dataset has been used in recent works on robust and verified perception \SC{CITE}.
Our prime goal is to test that we can build a perception model that performs well 

The X-plane public dataset has recently been used as a benchmark problem for the work on robust and verified perception CITE. This experiment demonstrates our method's performance on a much more challenging and realistic dataset. Importantly, we compare our method with standard single-step data augmentation techniques, the current state-of-the-art approach for generalized data augmentaion.

% \input{figures_latex/xplane_mpc}
% \input{figures_latex/xplane_wpt}


\subsubsection{Setting}

The input to our \SC{autonomous airplane (``robot'')} is a $128\times128$ RGB image $s$ of the scene, which is an image of the runway taken from the right wing. The \texttaskmodel \space $\alltaskmodel$ is a perception-planning module that outputs the current state of the airplane $\mathbf{w}_F$, given this sensory input $s$ and \SC{a} history \SC{of} waypoints $\mathbf{w}_P$. Specifically, the \texttaskmodel \space outputs \SC{a} single waypoint $\mathbf{w}_F$, which is a tuple of the distance
to the centerline of runway $y$ and the heading angle $\theta$, denoted by $w_F = {(y_i, \theta_i)}_{i=0}^{F},  F=1$. $ \mathbf{w}_P = {(y_i, \theta_i)}_{i=0}^{P}$ is a history of \SC{the} $P = 10$ past waypoints which are used to improve its predictions by the \texttaskmodel. The \texttaskcost \space is a standard quadratic tracking cost with linear dynamics constraints defined in Eq. \ref{eq:track_mpc}.

% It is important to note that in this setting, the \texttaskmodel only outputs the current state of the aeroplane. Tracking vector $\mathbf{w}_F$ for the mpc is a $F$ length vector of tuples $w_F = {(0, 0)}_{i=0}^{F}$, since we want the distance to the centerline and the headling angle to be 0. An example of the task scenario is shown in figure \ref{fig:xplane_scenario}. 

\paragraph*{Images from Diverse Weather Conditions: }
We will represent the whole X-plane dataset as $ \Gamma = \{ \datasetafternoon, \datasetmorning, \datasetovercast, \datasetnight \} $, where each dataset represents the corresponding subscript weather condition. Each individual weather dataset in $\Gamma$ has 44000 training scenarios and 11000 testing scenarios. The ground truth waypoint are part of dataset, obtained from the X-Plane simulator. 

We will compare 4 different \texttaskmodel $\mtaskmodel$, \textsc{Original} trained only on $\datasetafternoontrain$, \textsc{Data Added} trained on $\datasetaddtrain = \datasetafternoontrain \cup \datasetmorningtrain$ (afternoon and morning), \textsc{Data Augmentation} trained on $\datasetaugtrain = \datasetafternoontrain \cup \datasetaugtrain$ ($\datasetaugtrain$ created by performing image augmentations on $\datasetafternoontrain$) and \textsc{Task Driven} trained $\datasetafternoontrain \cup \datasetadvtrain$ ($\datasetadvtrain$ created using our method on $\datasetafternoontrain$). More details about datasets can be found in section \ref{sec:data_schemes}. We use $\datasetmorningtrain$ in $\datasetaddtrain$ since the morning and the afternoon weather conditions are very similar.

\input{figures_latex/xplane_metric}



This experiment shows that the \textsc{Task Driven} task model will have superior performance than the other \texttaskmodels \space on OOD $\datasetnighttest$ test datasets, specifically compared to the \textsc{Data Augmentation} task model. We quantitatively compare the performance of the above-mentioned \texttaskmodels \space on Average Task Cost $\taskcost$ and MSE for predicting the waypoints. We test these metrics on test datasets $\datasetafternoontest$, $\datasetmorningtest$, $\datasetnighttest$ and $\datasetadvtest$. 

\subsubsection{Quantitative results}
We quantitatively show that our scheme, \textsc{Task-Driven}, reduces the average \texttaskcost \space $\taskcost$, compared to other \texttaskmodels. Figure \ref{fig:xplane_mpc} (left) shows the average \texttaskcost \space (Y-axis in the fig.) for all the \texttaskmodels \space (shown in different colors in fig.) when evaluated on different \textit{test} data scenarios (X-axis in fig). On the $\datasetafternoontest$ and $\datasetmorningtest$, our \textsc{Task-Driven} scheme (red) performs on par with other \texttaskmodels. This is expected because all networks are trained on this data. Since the morning data is same as afternoon data, the \texttaskmodels \space perform similarly as well.
% The \texttaskmodel \textsc{Data Augmentation} is not able to help much since it is only creating single-step data augmentations, i.e. augmentation relevant only for perception \texttaskmodel but not for planning \texttaskmodel.

However, the key benefits of our approach are highlighted in the OOD test datasets $\datasetnighttest$ and $\datasetadvtest$. Our method of adversarial scenario generation automatically generates examples of challenging scenarios from the original $\datasetafternoontrain$ and adds them to $\datasetadvtrain$, making the \textsc{Task-Driven} \texttaskmodel \space robust to OOD test datapoints as shown in the \emph{night} and \emph{synthetic adversarial} columns in the figure \ref{fig:xplane_mpc}. The \textsc{Data Augmentation} \texttaskmodel \space cannot help that much since it only creates single-step data augmentations, i.e. augmentation relevant only for the perception \texttaskmodel \space but not for the planning \texttaskmodel. Our scheme, \textsc{Task-Driven}, has $28.2\%$ less average cost (Wilcoxon p-value of $0.0$) for the night test dataset and $16.6\%$ less average cost (Wilcoxon p-value of $0.0$) for the synthetic adversarial test dataset compared to \textsc{Data Augmentation}. 

%These differences are statistically significant with a  for the night test dataset and $0.0$ for the .

Figure \ref{fig:xplane_mpc} (right) shows how our \texttaskmodel, \textsc{Task-Driven}, achieves lower ultimate task cost by predicting future waypoints $\mathbf{w}_F$ correctly (measured by waypoint MSE). While all methods perform similarly on the original test dataset $\datasetafternoontest$, the key gains of our scheme are on the test datasets $\datasetnighttest$ and $\datasetadvtest$. Specifically, the \textsc{Task-Driven} scheme, has $54.7\%$ less average cost (Wilcoxon p-value of $0.0$) for the night test dataset and $42.6\%$ less average cost (Wilcoxon p-value of $0.0$) for the synthetic adversarial test dataset compared to \textsc{Data Augmentation}. 

\input{figures_latex/xplane_adv_scenario}

\textit{Qualitative Results: }
We now provide intuition for how the \textsc{Task-Driven} \texttaskmodel \space outperforms standard benchmarks by illustrating challenging adversarial scenarios that are automatically synthesized by our method in dataset $\datasetadvtrain$. Figure \ref{fig:adv_scenarios} shows two scenarios where our adversarial training scheme creates scenarios that make it that harder to detect the centerline on the runway. In the left of Fig. \ref{fig:adv_scenarios} the weather condition stays the same, but it is significantly harder to detect the centerline. In the right of Fig. \ref{fig:adv_scenarios} the adversarial training  changes the afternoon weather condition to night, which the \textsc{Original} \texttaskmodel \space has never seen before. Naturally, this increases the \texttaskcost \space since the \textsc{Original} \texttaskmodel \space has never seen these scenarios before. Rather than augmenting our dataset with well-understood scenarios already reflected in the training distribution, our scheme targetedly adds challenging scenarios that make the \textsc{Task-Driven} \texttaskmodel \space more robust. 



==> sections/intro.tex <==
Imagine a drone that must safely land on a variety of moving targets using its on-board camera and a learned perception module, such as a deep neural network (DNN). The drone's perception DNN, coupled with a downstream planning module, might output a sequence of waypoints to follow that
the drone can track using a model predictive controller (MPC). Ultimately, the drone's high-level task objective is to reduce control cost while following a safe trajectory. However, the drone will often operate in visual scenarios with radically different lighting, weather, and terrain conditions than its original training distribution. In this paper, we ask whether we can automatically synthesize adversarial visual scenarios for multi-step control tasks in order to re-train more robust robotic perception models.

Today, we can attempt to train robust perception models by methods including data augmentation, domain randomization, and synthesis of adversarial examples for single-step vision tasks. For example, data augmentation could add synthetic examples to a drone's visual training dataset by cropping images, randomly rotating them, or altering pixel hue. Likewise, we can alter selected pixels using adversarial attacks to change a perception model's classifications or object detections for \textit{single} time steps. However, these synthesized visual examples might be ultimately benign for an ultimate model-based controller, while other visual scenarios might directly affect key state estimates.  \textbf{Our key insight} is that we can characterize the sensitivity of (differentiable) MPC controllers to errors in waypoint predictions from planning modules, which can in turn be back-propagated to perception models to \textit{efficiently} learn adversarial visual scenarios that are most salient for control. Crucially, we can also synthesize those scenarios using \textbf{differentiable} rendering techniques, which map a set of latent parameters that describe a visual scene to a rendered visual input. 
In effect, by explicitly accounting for the ultimate task, we hypothesize we can more efficiently find adversarial visual examples to aid in robust re-training of perception models. 

%Our key observation is that a variety of robots are interfacing learned perception and planning DNNs with model-based controllers. Moreover, a variety of works have trained robust vision models for single-step inference tasks to guard against natural and synthetic adversarial visual perturbations or ``attacks''.
%However, it is still poorly understood how adversarial visual scenarios affect the ultimate multi-step control cost of MPC. 
%Then, if we re-train on these scenarios, we can develop more robust perception models that ultimately lead to lower control cost in the robotics pipeline. Crucially must be robust even as the  they operate in new lighting, weather, and terrain conditions far from their training distribution. Ultimately, the drone might use a model predictive controller (MPC) to track a waypoint that follows the trajectory, which leads to its final optimization objective of a control cost.

\textit{Literature Review: }
Our work is broadly related to adversarial training in machine learning (ML), data augmentation, differentiable model predictive control (MPC), and differentiable rendering methods. We now highlight how our approach differs from related work. 

It is well-known that many ML models are susceptible to adversarial examples. For example, in computer vision, methods can sublty alter selected pixels to produce wrong classifications from pre-trained vision models even though the perturbation is imperceptible to the human eye. These adversarial attacks, such as the popular Fast Gradient Sign Method (FGSM), essentially calculate the sensivity of a pre-trained classifer to distortions in the image input, which guides how we to make a bounded, adversarial perturbation to the original image. However, to the best of our knowledge, there is very little work on how such image perturbations affect \textit{multi-step, model-based} control tasks in robotics, such as navigation or control based on state estimates from deep perception models.

Our work is also related to data augmentation techniques, which add new synthetic examples to training datasets in order to increase their diversity and train more robust, generalizable ML models. However, our key observation is that today's data augmentation is largely task-agnostic -- we often do not add synthetic alterations to data that directly affect our ultimate task performance goal. For example, in computer vision, we might randomly crop, rotate, or alter the hue of pixels in attempt to train a more robust model. However, these perturbations could ultimately be benign for a downstream controller and thus data-inefficient to train upon. Instead, we should leverage the structure of a downstream control task to targetedly perturb pixels that are most salient for control and affect key state estimates for the controller. We note that the idea of task-driven data augmentation is in itself not new, and has been applied to augmenting datasets for graph neural networks (GNNs) etc. However, our key insight is to use recently-developed differentiable model predictive control (MPC) toolboxes to compute the sensitivity of a multi-step control task to pixel perturbations. 

\SC{adversarial control RL: \cite{lutter2021robust} focuses on RL being more robust

\cite{yang2021synthesis} focuses on safety specification violation

differentiable MPC: \cite{agrawal2020learningcontrol,agrawal2020learning,amos2018differentiable}

plain MPC: \cite{borrelli2017predictive,Camacho2013}

data augmentation: \cite{volpi2018generalizing}

AV space \cite{wang2021advsim}, uses Bayesian opt and LIDAR sensor failures. we look at diff MPC and gradient based approaches
another AV: \cite{feng2021intelligent}

Bayes Opt \cite{abeysirigoonawardena2019generating}

CV standard adv examples: \cite{goodfellow2014explaining,akhtar2018threat,hendrycks2021natural,xie2017adversarial}

domain randomization in robotics: \cite{tobin2017domain,tobin2018domain}

task-driven data augmentation \cite{zakharov2019deceptionnet,chaitanya2019semi}

X-Plane \cite{XPlane,taxinetDataset}

}

\textit{Contributions and Organization: }
In light of prior work, our contributions are three-fold. 
\begin{itemize}
    \item First, we present a method to automatically synthesize adversarial examples for data-driven perception models that directly affect a model-based controller's ultimate cost. 
    \item Second, we develop a novel loss function that flexibly trades-off the realism of adversarial examples with their impact on control cost. Specifically, we learn perturbations in a latent space that generates visual scenes and quantify that the rendered scenes are similar to historical data yet poor for control.
    \item Third, we show that re-training on these synthesized examples leads to better performance on unseen test data than today's standard task-agnostic data augmentation methods. We demonstrate this result on a challenging scenario where an aircraft must taxi on a runway using an on-board vision model in a photo-realistic simulator.
\end{itemize}

\textit{Paper Organization: }



==> sections/method.tex <==
\subsection{Problem Statement}

\input{figures_latex/architecture}

Fig. \ref{fig:expr_arch} shows a typical robotic learning system consisting of a \texttaskmodel \space and a \texttaskcost. In the case of self-driving cars, the \texttaskmodel \space consists of a perception module $\mpercep$ which takes sensory information of the scene, such as images or LiDAR, as inputs and derives a latent representation of the scene. The planning module $\mplan$ uses the latent representation to generate a safe and comfortable waypoint trajectory. The \texttaskcost \space is usually the motion planning cost. Thus, unsafe and aggressive waypoint trajectories are assigned higher costs, while safe and smooth trajectories are assigned lower costs. Next, we formally define the \texttaskmodel \space and the \texttaskcost.

\textit{Task Model:} The goal of the \texttaskmodel \space is to understand the robot's environment and generate future actions for the robot to achieve a specific task. We consider one of the most general \texttaskmodels, consisting of a perception module $\mpercep$ and a planning module $\mplan$. The perception module understands the environment around the robot by taking the sensory inputs from the environment. Specifically, the perception module $z = \mpercep (s)$  takes an image $s$ of the scene as input and outputs a latent representation $z$ of the scene. The planning module estimates the robot's current state and generates future actions for the robot. The planning module,$\mathbf{w}_F = \mplan(z, \mathbf{w}_P)$, takes the latent representation $z$ of the scene and a vector of the robot's past waypoints $\mathbf{w}_P$ as input and outputs a vector of future waypoints $\mathbf{w}_F$ for the robot to follow ($P$, $F$ is the number of waypoints). The waypoints $\mathbf{w}_P$ (or $\mathbf{w}_F$) are a sequence of $P$ (or $F$) tuples consisting of the robot's state. Robot's state is defined by the user for the specific use-case, for eg. $\mathbf{w}_P = \{ l_x, l_y, v, \theta \}_{i=1}^{P}$, where $l_x$ and $l_y$ are the robot's $x,y$ location in meters, $v$ is the speed in meters/sec and $\theta$ is robot's angle in radians. We will represent the whole \texttaskmodel, $\alltaskmodel$, by $\mtaskmodel$.

\textit{Task Cost:} To quantify the quality of the predicted waypoints by the \texttaskmodel, we use the \texttaskcost. The \texttaskcost, $\taskcost( \mathbf{w}_F ) \in \mathbb{R} $, measures the quality of $\mathbf{w}_F$ (the waypoints predicted by the \texttaskmodel) as a scalar value. For eg. the \texttaskcost \space could either measure smoothness of predicted waypoints $\mathbf{w}_F $, how much extra control will be utilized to execute waypoints $\mathbf{w}_F $ or check if the waypoints $\mathbf{w}_F$ violate the physical limits of the robot, etc. Therefore, undesired waypoints, $\mathbf{w}_F $, will have higher cost and vice versa. In this work, we will assume that $\taskcost$ is differentiable. 

%% The waypoints $\mathbf{w}_P$ ( or $\mathbf{w}_F$ ) are a sequence of P (or F) tuples consisting of $(x,y)$ locations of the robot, denoted by $\mathbf{w}_P = {(x_i, y_i)}_{i=0}^{P}$ (or F)
\textit{Differentiable Rendering Module:} \label{sec:diff_rendr_module}
In order to parametrize the input scenes, $s$, we introduce a differentiable rendering module $\render$. The differentiable rendering module, $ s = \render(\nu)$, generates the robot's scene input $s$ with the parameters $\nu$ and builds a latent space of the \texttaskmodel \space inputs, $s$, by parametrizing them with $\nu$. Therefore, the differentiable rendering module provides us with an ability to generate new scenes from the latent space. In our setting, $\render$ is a Decoder from a Variational Auto Encoder (CITE), described in section \ref{sec:expr_prelim}.

\textit{End-to-End Differentiable System:}
Using a differentiable \texttaskcost \space and a differentiable rendering module ($\render$) enables us to create an end-to-end differentiable mapping from input scene parameters, $\nu$, to the final \texttaskcost, as shown in Fig. \ref{fig:expr_arch}. This end-to-end differentiable mapping can be leveraged to back-propagate based on the final \texttaskcost \space w.r.t. to input scene parameters $\nu$. We use the differentiable rendering module to synthesize new scene inputs, $\bar{s}$, with a higher \texttaskcost \space compared to the original input scene $s$, we discuss this process in detail in section \ref{sec:method_setting} and Algorithm \ref{alg:train}.

\textit{The Problem:} A dataset, $\dataset$, containing $N$ tuples of inputs $x$ and ground-truth labels $y$ is denoted by $\datasetall$. For each $n \in N$, we have $x^{(n)} = \{s, \mathbf{w}_P\}$, the input scenes and past waypoints respectively. Similarly, we have $y^{(n)} = \{\mathbf{w}_F\}$ the future waypoints as labels. The dataset, $\dataset$, is separated into train dataset, $\datasettrain$ and a held-out test dataset, $\datasettest$. We train a \texttaskmodel \space on the train dataset, $\datasettrain$, to predict future waypoints, $\mathbf{w}_F$, given inputs $\{s, \mathbf{w}_P\}$. The \texttaskmodel \space trained on the dataset, $\datasettrain$, is represented as $\mtaskmodeldataset$. In a typical robot-learning system, we want the waypoints, $\mathbf{w}_F $ , predicted by $\mtaskmodeldataset$ to have lower \texttaskcost \space and also be robust to unseen scenarios, i.e. have good performance on the held-out dataset $\datasettest$. The problem we are tackling is what additional dataset $\datasetnewall$ with $M$ datapoints we can add to original dataset $\dataset$, such that a \texttaskmodel \space trained on combined dataset, $\dataset \cup \datasetnew$ will have a lower \texttaskcost \space and perform better on the held-out test dataset, $\datasettest$, compared to the original \texttaskmodel, $\mtaskmodeldataset$.  

% Specifically, each example $x = (s, \mathbf{w}_P)$ represents robot's image scene input $s$ and the history of waypoints $\mathbf{w}_P$. Using the inputs $x$, the \texttaskmodel \space predicts a ground-truth target vector $y = (\mathbf{w}_F)$ which represents the future waypoints for the robot to follow. 

% We experimentally show that a \texttaskmodel \mtaskmodel trained on the combined dataset \dataset $\cup$ \advdataset will have a lower average \texttaskcost \taskcost and will be more robust compared to a \texttaskmodel \mtaskmodel trained with standard single-level data augmentation techniques on out-of-distribution data. 

% Additionally, the new  \texttaskmodel \space will be more robust to out-of-distribution datapoints $ ( x^{'}, y^{'}) \notin$ \dataset $\cup$ \advdataset.

\subsection{Proposed Method} \label{sec:method_setting}
We hypothesize that we can significantly improve the task model if we re-train it on a dataset that includes scenarios where the original task model performs poorly. Thus, our goal is to synthetically generate adversarial scenarios for the original task model which lead to high task cost (i.e. poor performance). Our proposed method generates a new adversarial dataset $\advdatasetall$ from a given original $\dataset$, such that the original \texttaskmodel, $\mtaskmodeldataset$, will have a higher \texttaskcost \space $\taskcost( \hat{y} )$ for the new dataset $\advdataset$. 

To do so, we introduce the notion of a differentiable adversary to generate the new dataset $\advdataset$, shown in orange in Fig. \ref{fig:expr_arch}. Informally, the adversary finds new scene inputs $s$ for the \texttaskmodel \space that increase the \texttaskcost. We represent the adversary as $\adv(  \nu ;\advparam ) $, where $\nu$ is the input which we want to make adversarial and $\advparam$ are $\adv$'s trainable parameters. Adversary $\adv$ will generate adversarial output $\bar{\nu}$ from input $\nu$, represented as $ \bar{\nu} = \adv(\nu; \advparam) $, under the defined task cost $\taskcost$.

\textit{Adversary Loss Function:} The adversary, $\adv$, is trained using loss function $\loss$ defined in \eqref{eq:adv_loss}. Intuitively, the adversary loss function $\loss$ needs to increase the \texttaskcost \space by generating $\bar{\nu}$, while also making sure that $\bar{\nu}$ is realistic and thus close to $\nu$. Therefore, the adversary loss function (\eqref{eq:adv_loss}) has two main terms, the differentiable \texttaskcost \space and distance loss between $\bar{\nu}$ and $\nu$. 

% We additionally add the regularization term to the adversary loss function $L ( \bar{\nu}, \advparam )$ to make sure the adversarial parameters not blow up.


We adversarially generate $\bar{\nu}$ from the adversary $ \bar{\nu} = \adv(\nu; \advparam) $, where $\nu$ are scene $s$'s original latent representation in differentiable rendering module $\render$. Thus, $\bar{\nu}$ is the adversarially generated latent representation of scene $s$. We then generate new scene $\bar{s}$ using differential renderer $\render$, $\bar{s} = \render(\bar{\nu})$. Next, we get a new output waypoint prediction $\mathbf{w}_F$ using the \texttaskmodel $\mtaskmodel$ for the adversarial scene $\bar{s}$, $\mathbf{w}_F = \mplan(\bar{s}, \mathbf{w}_P)$. Finally, we calculate the new \texttaskcost \space $\taskcost$,  $ \taskcost( \mathbf{w}_F )$.


% In equation \ref{eq:adv_loss}, $\hat{J}(  \nu, \advparam )$ is defined in Equation \ref{eq:adv_loss_J} Equation \ref{eq:adv_loss_J} calculates the cost of adversarial input $\bar{x}$ generated using parameters adversarial parameters $\bar {\nu}$. All the transformations from equation \ref{eq:adv_loss_J_adv} to equation \ref{eq:adv_loss_J_cost}, can are presented in 1 step in equation  \ref{eq:adv_loss_J_all}.

% \begin{subequations} \label{eq:adv_loss_J}
% \begin{align}
%     \text{Generate  Differentiable} & \text{ Render parameters} \nonumber \\ 
%   \bar {\theta} &= f( \theta; \advparam)   \label{eq:adv_loss_J_adv}  \\
%   \text{Generate new data input}  \nonumber \\
%   \bar{x} &= \psi(\bar{\theta}) \ \label{eq:adv_loss_J_render} \\
%   \text{Make new task prediction} \nonumber \\
%   \bar{y} &= \Phi_n (\bar{x})  \label{eq:adv_loss_J_model} \\
%   \text{Calculate Task Loss}  \nonumber\\
%   \hat{J}(  \theta, \advparam ) &= J(\bar{y}) \label{eq:adv_loss_J_cost} \\
%   \nonumber \\
%   \hat{J}(  \theta, \advparam ) &= J( \Phi_n ( \psi( f( \theta) ) ) ) & \label{eq:adv_loss_J_all}
% \end{align}
% \end{subequations}

One of the key problem associated with adversarial scenario generation, is generating scenarios, $\bar{s}$, which are realistic and can occur in real-world. Generating scenarios which are not realistic might not help in improving the \texttaskmodel's robustness, as the \texttaskmodel \space will never have to deal with those scenarios. Therefore we add a distance loss $\distloss \in \mathbb{R}$. The distance loss measures the distance between the original input $s$ and the adversarially generated scene $\bar{s}$ in the latent space of $\render$. Calculating the distance loss in the latent space is a novelty of our loss function, based on the observation that similar scenes $s$ and $\bar{s}$ might be very far in the high-dimensional image space but might be close in the latent space of the renderer $\render$. Specifically, we calculate the distance loss $\distloss$ between latent space variables $\nu$ and $\bar{\nu}$, instead of the actual scene $s$ and $\bar{s}$. The distance loss $\mathcal{I}$ is weighted by $\kappa$ in the optimization step, which controls how much we allow $\bar{s}$ to deviate from $s$. We use the L2-norm for the distance loss, actual implementation is discussed in section \ref{sec:expr_prelim}.

\begin{equation} \label{eq:adv_loss}
\begin{aligned}
  \loss = \hat{J}( \bar{\nu}, \advparam )  \mathbf{-} \kappa \distloss
  % \max_{\advparam} L ( \bar{\nu}, \advparam ) = \hat{J}( \bar{\nu}, \advparam )  \mathbf{-} \kappa \distloss \mathbf{-} \lambda ||\advparam||_{p} 
\end{aligned}
\end{equation}

\textit{Adversary Training:} Algorithm \ref{alg:train} shows the complete adversary training procedure. We iterate over each datapoint and save the most adversarial synthetic examples generated by the adversarial input using an adversary $\adv$. In order to generate the most adversarial synthetic examples, we decided to use a new adversary for each datapoint rather than training a common adversary for the whole dataset. 

Starting from line 2, we sequentially iterate through the original dataset $\dataset$. We obtain the latent space representation $\nu_i$ of the datapoint $x_i$ from the differential renderer $\render$ in line 3. In line 4, we initialize a new adversary $\adv$ with random weights $\advparam_{k=0}$, which will be specific to the datapoint $x_i$. Then, we iterate for $K$ gradient descent steps, indexing the weights $\advparam$ and the generated latent variable $\bar{\nu}$ by $k$. Finally, in lines 5-7, we initialize the latent variable $\nu_{k}$, best task cost $J^{\star}$ and the adversary tuple $(\bar{x}, \bar{y}, \bar{\nu})$.

In lines 8-18, we perform $K$ gradient update steps to train the adversary $\adv$. In each gradient step $k$, we update the adversary parameters to $\advparam_{k}$ using adversary loss function $ L ( \bar{\nu}_{k},\advparam_{k-1} ) $ and back-propagation (lines 10-13). In lines 14-18, we store the adversarial tuple $( \bar{x}_k , y_i, \bar{\nu_{k}} ) $ if it has higher Task Cost $\hat{J}( \bar{\nu_{k}},  \advparam_{k} )$ than the previous best \texttaskcost \space $J^{\star}$. Finally, after $K$ gradient steps, we append the best adversarial datapoint $ (\bar{x}, \bar{y}, \bar{\nu}) $ to dataset $\advdataset$ in line 19. It is important to note that we keep all the network weights frozen during adversarial training, and only adversary parameters $\advparam$ are updated.

\begin{small}
\begin{algorithm}[t]
\DontPrintSemicolon
\SetNoFillComment % <---------------------------
\SetAlgoLined
Initialize new dataset $\advdataset$  \; 
\For{$ (x_i, y_i) \gets$  $\datasetall$,  $0 \leq i \leq N$ }{
  Get $x_i$'s differential renderer params $\nu_i$ \;
  Init adver $\adv( \nu_i ; \advparam_{k=0} ) $ with random $\advparam_{k=0}$   \;
  $\bar{\nu}_{k =0 } = \nu_i  $ \;
  Best Task Loss $ J^{\star}  = - \infty $ \;
  Initialize Adversary Tuple = $(\bar{x}, \bar{y}, \bar{\nu})$ \;
  \For{$k~ \gets 1 $ \KwTo K } {
    % $\bar{x_k} = \psi( \bar{\nu_{k}} )$ \;
    % $\bar{y_k} = \Phi_n (\bar{x_k})$ \;
    % $\hat{J}(  \bar{\nu_{k}}, {\advparam_{k}}^i ) = J(\bar{y_k}$ ) \;
    $ \bar{\nu}_{k} = \adv(  \bar{\nu}_{k - 1}  ; \advparam_{k-1} )  $ \;
    Calculate \texttaskcost \space $\hat{J}( \bar{\nu}_{k},  \advparam_{k-1} )$ \;
    Calculate Loss:  $ L ( \bar{\nu}_{k},\advparam_{k-1} ) $  \;
    Calculate gradient $\nabla g = \nabla_{\advparam_{k-1}}  L ( \bar{\nu}_{k}, \advparam_{k-1} )$ \;
    Update params to $ \advparam_{k} $ from $ \advparam_{k-1} $  \;
    % Update params to $ \advparam_{k} $ from $ \advparam_{k-1}+ \alpha \nabla g $  \;
    
    % $ \advparam_{k + 1}^i = f(\bar{\nu_{k}}; \advparam_{k}^i )$ \;
    \If{ $\hat{J}( \bar{\nu_{k}},  \advparam_{k-1} ) \geq J^{\star}$   } {
        $ (\bar{x}, \bar{y}, \bar{\nu}) = ( \bar{x}_k , y_i, \bar{\nu_{k}} ) $  \;
        $ J^{\star} \gets \hat{J} $ \;
    }
    }
    Append $ (\bar{x}, \bar{y}, \bar{\nu}) $ to  $\advdataset$ \;
 } \caption{\textbf{Adversary Training}}
 \label{alg:train}
\end{algorithm}
\end{small}


We experimentally show that a \texttaskmodel \space $\mtaskmodel$ trained on the combined dataset $\dataset$ $\cup$ $\advdataset$ will have a lower average \texttaskcost \space $\taskcost$ and will be more robust compared to a \texttaskmodel \space $\mtaskmodel$ trained with standard single-level data augmentation techniques on out-of-distribution data. 



%%%%%%%%%%%%%%%%%%%%%%%%

% Finally, we regularize the adversary parameters $\advparam$ with a q-norm $||\advparam||_{q} \in \mathbb{R}$ term, weighted by $\lambda$. Since we are maximizing the loss function in equation \ref{eq:adv_loss}, the distance loss and regularizer are subtracted.

% \subsection{Adversary Training} \label{sec:adv_training}
% We train our adversary using standard gradient descent. We update adversary parameters at each gradient step $k$ using the update equation \ref{eq:adv_grad}. $\Pi_{\advparam}$ is the Euclidean projection operator onto the set of allowable parameter space $\advparam$. $\alpha > 0$ is the gradient step size. Since we are maximizing the loss in equation \ref{eq:adv_loss}, we are adding gradients in equation \ref{eq:adv_grad}.

% \begin{equation} \label{eq:adv_grad}
% \begin{aligned} 
%   \advparam_{k} = \Pi_{\advparam}\left(\advparam_{k-1} + \alpha \nabla_{\advparam}  L ( \bar{\nu}, \advparam_{k-1} ) \right)
% \end{aligned}
% \end{equation}
% Adversary loss $L$ gradient w.r.t to adversary parameters $\advparam$ is shown in equation \ref{eq:adv_grad_gradient}.

% For each input $x$ and its corresponding parameters $\theta$, we train a new adversary $\adv( \cdot \hspace{1.0mm} ; \advparam ) $, using gradient descent as show in Equation \ref{eq:adv_grad}.  $\nabla g$ in equation \ref{eq:adv_grad_gradient} is the gradient of loss in equation \ref{eq:adv_loss} w.r.t to adversary parameters $\advparam$. 

    % \nabla_{\advparam}  L ( x, \theta, \advparam ) &= \frac{\partial \hat{J}(  \theta, \advparam )}{\partial \advparam} - \kappa \cdot\frac{\partial \mathcal{I}(x, \bar{x}) }{\partial \advparam}  - \lambda  \cdot \frac{\partial ||\advparam||_{p} }{\partial \advparam } \label{eq:adv_grad_gradient} \\
% \nabla_{\advparam}  L ( x, \theta, \advparam ) &= \frac{\partial \hat{J}(  \theta, \advparam )}{\partial \theta} \cdot \frac{\partial \theta}{\partial f } \cdot \frac{\partial f}{\partial \advparam } - \kappa \cdot\frac{\partial \mathcal{I}(x, \bar{x}) }{\partial f} \cdot  \frac{\partial f}{\partial \advparam } - \lambda  \cdot \frac{\partial ||\advparam||_{p} }{\partial \advparam }


==> sections/sandeep_edits/RSS21_problem_statement.tex <==
\revision{We now introduce the core compute modules for information flow between a robot and a central server (Fig. \ref{fig:task_autoencoder}), and then formalize our problem statement}. \revision{First, a robot measures a sensory input $x \in \reals^n$, such as an image or LIDAR point cloud. Without loss of generality, $x$ could represent a single sensory sample a robot wishes to transmit or a window $w$ of correlated samples measured from time $t-w$ to $t$, such as a segment of video, denoted by $\mathbf{x}= x^{t-w:t}$.} 

\noindent \tu{Robot Encoder:}
The encoder maps raw input $x$ to a concise representation  $z \in \reals^\zbottleneck$, denoted by \RSS{$z = \fencoder(z | x; \thetaencoder)$}, \revision{where $\thetaencoder$ are encoder model parameters, such as learned DNN weights}. Henceforth, $z$ is referred to as a bottleneck representation, since it is compressed via an information bottleneck, such as a DNN hidden layer, to a size $\zbottleneck \ll n$. 

\noindent \tu{Server Decoder:}
The encoder transmits bottleneck representation $z$ over a wireless link to a differentiable decoder at a central server, which generates a reconstructed estimate of the raw sensory input \RSS{$\xhat = \fdecoder(x | z; \thetadecoder)$}. \revision{The parameters of a decoder model, such as a DNN, are denoted by $\thetadecoder$}. 

\noindent \tu{Server Task Network:}
Finally, the decoded input $\xhat$ is \textit{directly passed} through a pre-trained, differentiable task module, which serves as the key distinction of our work from a standard autoencoder. \revision{An example} of a task module could be a DNN object detector that predicts object locations and classes $\yhat = \ftask(\xhat; \thetatask)$ using model parameters $\thetatask$. Crucially, by decoding to the original input dimension $n$, our approach enables robots to directly utilize a plethora of pre-trained, publicly-available task modules that expect an input dimension $n$ without re-training on custom bottleneck representations $z$.
In practice, the encoder, decoder, and task module can all be DNNs. We assume sensory input $x$ and its label $y$ are drawn from a domain-specific distribution $\mathcal{D}$, such as the space of all Mars terrain images and labels. 

\subsection{Task and Reconstruction Optimization Objectives}
Our principal objective is to minimize the {\em task loss} $\taskloss(y, \yhat; \thetatask)$, which compares the resultant task outputs $y = f(x; \thetatask)$  using original input $x$ and predicted outputs $\yhat = \ftask(\xhat; \thetatask)$ using a decoded input $\xhat$. Our key technical insight is that robotic perception tasks can often tolerate considerable distortion in the input estimate $\xhat$, such as omitting irrelevant parts of an image/map for classification/planning, as long as the downstream task module $\ftask(; \thetatask)$ can still achieve its goal. \revision{Thus, decoded input $\xhat$ should only represent task-relevant features, which enables highly-compressed representations $z$ to be transmitted over a wireless link}.

Optionally, a roboticist might want to also minimize reconstruction loss, in cases where decoded inputs $\xhat$ should be moderately human-interpretable to view or debug portions of an image. For such scenarios, loss function $\reconloss(x, \xhat; \thetaencoder, \thetadecoder)$ incentivizes faithful reconstruction of a scene, which, in practice, could be the standard variational autoencoder regularized loss \cite{kingma2013auto}. We provide a general, flexible co-design framework that allows a roboticist to optimize a weighted combination of task and reconstruction loss, with reconstruction loss weight $\lambda \ge 0$: 
\vspace{-1em}

\begin{small}
\begin{align}
    \weightedloss(x,\xhat, y, \yhat; \thetatask, \thetaencoder, \thetadecoder) = \nonumber \\ \taskloss (y, \yhat; \thetatask) + \lambda \reconloss (x, \xhat; \thetaencoder, \thetadecoder). 
\label{eq:weighted_loss}
\end{align}
\end{small}
Our experiments evaluate the scenario of strictly optimizing for task loss ($\lambda=0$) as well as various values of $\lambda > 0$, which introduces a regularization term to incentivize highly-compressed representations that still yield human-interpretable reconstructions. Having defined our optimization objective, we now formalize our problem statement. 

\subsection{Problem Statement}
\begin{problem}[Sensory Co-design for Machine Perception]
\label{prob:codesign}
Given a differentiable task module $f(; \thetatask)$ with fixed, pre-trained parameters $\thetatask$, fixed bottleneck dimension $\zbottleneck$, and reconstruction loss weight $\lambda \geq 0$, find robot encoder and server decoder parameters $\thetaencoder$ and $\thetadecoder$ that minimize weighted loss (Eq. \ref{eq:weighted_loss}) over data distribution $\mathcal{D}$:\vspace{-1em}

    \begin{small}
    \begin{align*}
        \thetaencoder^{*}, \thetadecoder^{*} = \argmin_{\thetaencoder, \thetadecoder} \mathop{\mathbb{E}}_{(x,y)\sim \mathcal{D}} \weightedloss (x, \xhat, y, \yhat; \thetatask, \thetaencoder, \thetadecoder), 
    \end{align*}
    \end{small}
    where $\xhat = \fdecoder(\fencoder(x; \thetaencoder); \thetadecoder)$ and $\yhat = \ftask(\xhat;\thetatask)$.
\end{problem}

% why does the problem matter?
\revision{Prob. \ref{prob:codesign} is widely applicable to resource-limited robots, such as space and mining rovers, that can unlock large benefits of remote computation if they send \textit{task-relevant} information over a bandwidth-limited network. The key novelty of our formulation is that we leverage knowledge of a task objective, through $\ftask(;\thetatask)$, to guide task-relevant representation learning of encoder/decoder parameters $\thetaencoder, \thetadecoder$. \RSS{Our formulation is related to multi-task learning for vision, which often considers semantically-similar tasks, such as segmentation and object detection \cite{crawshaw2020multi}. In contrast, however, our weighted objective has two semantically-different (and often competing) goals of learning a sparse set of features for machine perception while also regularizing for pixel-wise reconstruction for human-interpretability.}
    %\RSS{While our use of a weighted objective for reconstruction and machine perception is reminiscent of multi-task learning, our work differs since we are optimizing a communication scheme
Further, we enable a roboticist to set bottleneck size $\zbottleneck$ in a precise manner based on a network's maximum allowable data-rate. For example, the data-rate could be the size of $Z$ 32-bit floating point values sent at a certain communication frequency.}

\subsection{Illustrative Example: Linear Systems Setting}
\label{subsec:linear_setup}
To illustrate the compression benefits of optimizing for task loss in Prob. \ref{prob:codesign}, we consider a toy example where the encoder, decoder, and task module are matrices.
\revision{Specifically, consider a simple robotic sensor network where a central server must estimate a function $y = \KLQR x$ of a potentially large sensor measurement $x$, \textit{without} necessarily sending the full input $x$ over a wireless link.}
First, robot encoder matrix $\Aencoder = \thetaencoder \in \reals^{\zbottleneck \times \ninput}$ generates encoding $z = \fencoder(x; \thetaencoder) = \Aencoder x$. After $z$ is sent over a wireless link, it is decoded to $\xhat = \fdecoder(z; \thetadecoder) = \Bdecoder z$ by linear decoder $\Bdecoder = \thetadecoder \in \reals^{\ninput \times \zbottleneck}$. Finally, task matrix $\KLQR \in \reals^{\moutput \times \ninput}$ generates the output of the linear estimation problem $y \in \reals^\moutput$. 
\revision{The task loss penalizes error in the linear estimate $y=\KLQR x$, and the reconstruction loss optionally penalizes error in the sensor estimate $\xhat$ in case elements of $\xhat$ need to be sanity-checked. Both the task and reconstruction loss are quadratic, yielding weighted loss:}
\begin{align}
    \weightedloss = \underbrace{\Vert (\KLQR x - \KLQR \Bdecoder \Aencoder x) \Vert^2_2}_{\mathrm{task~loss}} + \lambda \underbrace{\Vert(\reconoperand)\Vert^2_2}_{\mathrm{recon. loss}}.
    \label{eq:weighted_loss_linear}
\end{align}
To show the full benefits of task-based compression, we now provide an analytical solution for Prob. \ref{prob:codesign} for the special case when $\lambda=0$ (pure task loss objective).
\noindent \begin{thm}[Linear Task-Aware Compression]
Consider task matrix $\KLQR \in \reals^{\moutput \times \ninput}$ with rank $r$ and compact singular value decomposition (SVD) $K = U \Sigma V^{\trans}$, where $U\in\reals^{\moutput \times r}$ and $V^{\trans} \in \reals^{r \times n}$ are semi-unitary.
Then, for bottleneck dimension $r$, setting $\Aencoder = V^{\trans}$ and $\Bdecoder = V$ solves Prob. \ref{prob:codesign} with zero task loss $\Vert (\KLQR x - \KLQR \Bdecoder \Aencoder x) \Vert^2_2$ (Eq. \ref{eq:weighted_loss_linear} with $\lambda=0$) for any $x \in \reals^{n}$. 
Further, there are no encoder and decoder matrices with bottleneck $Z < r$ that achieve zero task loss.
\end{thm}
\noindent \begin{proof}
The task loss is zero when, for any $x \in \reals^{\ninput}$, $y = \KLQR x = \yhat = \KLQR \Bdecoder \Aencoder x$. This is achieved when $\Bdecoder = V$ and $\Aencoder = V^{\trans}$:
\begin{small}
\begin{align*}
    \yhat = \KLQR \Bdecoder \Aencoder x &= \underbrace{(U \Sigma V^{\trans})}_{SVD(K)} \times \underbrace{V}_{\Bdecoder} \times \underbrace{V^{\trans}}_{\Aencoder} \times x \\
							&= U \Sigma V^{\trans} x = Kx = y,  
\end{align*}
\end{small}
\vspace{-1em}

\noindent where $V^{\trans}V = I_{r \times r}$ since $V$ is semi-unitary. We now show there are no other solutions with bottleneck $Z< r$. For the sake of contradiction, suppose there exist $\Atilde\in\reals^{Z\times n}, \Btilde \in \reals^{n\times Z}$ with $Z < r$ that achieve zero task loss. Then:
\begin{small}
\begin{align*}
    \text{rank}(\Btilde\Atilde) \leq ~&\text{min}(\text{rank}(\Atilde), \text{rank}(\Btilde)) \leq Z, \text{and} \\ 
    \text{rank}(\KLQR\Btilde\Atilde) \leq ~&\text{min}(\text{rank}(K), \text{rank}(\Btilde\Atilde)) \leq Z.
\end{align*}
\end{small}
However, in order for $\Atilde, \Btilde$ to achieve zero task loss, we must have $Kx=K\Btilde\Atilde x$ for any $x \in \reals^{\ninput}$, meaning we must have $K = K\Btilde\Atilde$. However, this is a contradiction since $\text{rank}(K\Btilde\Atilde)\leq Z < r=\text{rank}(K)$. Thus, we conclude there are no solutions that achieve zero task loss for $Z < r$.
\end{proof} 

\tu{Compression benefits:}
Our key insight is that, by co-designing with fixed task matrix $\KLQR$, we achieve zero task loss with a compression gain of $\frac{n}{\text{rank}(K)}$ compared to sending full input $x$. However, we do not necessarily have zero \textit{reconstruction loss} since matrix $V^{\trans}$ is only semi-unitary, meaning it is not required for $V V^{\trans} = \Bdecoder \Aencoder$ to be an identity matrix. \SC{In fact, if we want zero reconstruction loss, then we have $\hat{x} = \Bdecoder \Aencoder x= x$ only when $\Bdecoder = \Aencoder^{-1}$, requiring $\Bdecoder$ and $\Aencoder$ to be square $n \times n$ matrices, yielding no compression gain.} Crucially, our solution differs from na\"ively just computing $y=Kx$ directly at the robot, since we only transmit a small representation $z=V^{\trans}x$ and use the modular task matrix $\KLQR$ at the server. Finally, we note that the choice of $A=V^{\trans}$ and $B=V$ is not unique for bottleneck $r$. For example, we can scale the encoder to $aA$ and decoder to $bB$ where $ab=1$.

\subsection{Illustrative Example: Weighted Linear Setting}
We now generalize our previous result for the \textit{weighted} linear setting with $\lambda > 0$.
The key highlight of our solution is that the optimal linear encoder/decoder to minimize weighted task loss are simply a solution to a low-rank approximation problem. To establish this result, we first
concatenate $N$ examples drawn from training dataset $(x,y) \sim \mathcal{D}$ into a sample matrix $\bold{X} \in \reals^{n \times N}$. Given the dataset $\bold{X}$ and a bottleneck constraint $Z$, minimizing the weighted task loss (Eq. \ref{eq:weighted_loss_linear}) in the linear setting amounts to solving: 
\begin{small}
\begin{align}
    \argmin_{A,B} & \sum_{i=1}^{N}(\hat{\bold{X}}_i - \bold{X}_i)^\top (K^\top K + \lambda I)(\hat{\bold{X}}_i - \bold{X}_i)
    \quad{\text{~where~}} \notag \\
    & \hat{\bold{X}} = BA \bold{X}, ~\text{rank}(B) \le \zbottleneck \text{~and~rank}(A) \le \zbottleneck. 
    \label{eq:low_rank_approximation}
\end{align}
\end{small}
In the above problem, the $i$-th column of $\bold{X}$ and $\hat{\bold{X}}$ are given by $\bold{X}_i$ and $\hat{\bold{X}}_i$ respectively.
The following theorem solves Problem 1 for the weighted linear setting (Eq. \ref{eq:weighted_loss_linear}) by reducing it to a canonical low-rank approximation problem.

\begin{thm}[Linear Weighted Compression]
    The linear setting of Problem 1 is a canonical low-rank approximation problem with an analytical solution for an optimal encoder matrix $A$ and decoder matrix $B$.
\end{thm}

\begin{proof} (Sketch) 
    \renewcommand{\qedsymbol}{}
    %We first note that the matrix $K^\top K + \lambda I$ is symmetric and positive semi-definite and denote its eigen-decomposition by $Y \Lambda Y^\top$. 
    We first note that the real matrix $K^\top K + \lambda I$ is positive semi-definite, which admits an eigen-decomposition denoted by $Y \Lambda Y^\top$, where $Y$ is orthogonal. 
    Denoting the Frobenius norm of a matrix as $\doublevert \cdot \doublevert_F$, we can write the weighted task loss for Problem 1 in the linear setting as:
    \begin{small}
    \begin{align*}
        & \sum_{i=1}^{N}(\boldXhat_i - \boldX_i)^\top (K^\top K + \lambda I) (\boldXhat_i - \boldX_i) \\
    = & \sum_{i=1}^{N}(\boldXhat_i - \boldX_i)^\top (Y \Lambda Y^\top) (\boldXhat_i - \boldX_i) \\ 
    = & \doublevert \Lambda^{\frac{1}{2}} Y^\top \boldXhat - \Lambda^{\frac{1}{2}}Y^\top \boldX \doublevert_F^2.
    \end{align*}
    \end{small}
    Thus, the solution to Problem 1 with a bottleneck $Z$ in the linear setting can be written in the following low-rank approximation form: 
    \begin{small}
    \begin{align}
        \argmin_{A,B} \doublevert \underbrace{\Lambda^{\frac{1}{2}}Y^\top BA \boldX}_{\mathrm{approximation}} - \underbrace{\Lambda^{\frac{1}{2}}Y^\top \boldX}_{\mathrm{original}} \doublevert_F^2 \quad{\text{~where~}} \notag \\
        ~\text{rank}(B) \le \zbottleneck \text{~and~rank}(A) \le \zbottleneck. 
        \label{eq:low_rank_approximation_final}
    \end{align}
    \end{small}
    Thus, as stipulated by the Eckhart-Young theorem, the solution to Eq. \ref{eq:low_rank_approximation_final} is the rank $Z$ truncated singular value decomposition (SVD) of matrix $\Lambda^{\frac{1}{2}}Y^\top\boldX$, denoted by $U \Sigma V^\top$. For the SVD, $U\in\reals^{n \times Z}$ is semi-orthogonal, $V \in \reals^{N \times Z}$ is semi-orthogonal, and $\Sigma \in \reals^{Z\times Z}$ represents a diagonal matrix of singular values. Thus, an encoder of $A = U^\top \Lambda^{\frac{1}{2}} Y^\top$ and decoder of $B = (\Lambda^{\frac{1}{2}} Y^\top)^{-1}U$ are solutions since:
\begin{small}
\begin{align*}
    \underbrace{\Lambda^{\frac{1}{2}}Y^\top BA \boldX}_{\mathrm{approximation}}
    = & ~\Lambda^{\frac{1}{2}}Y^\top \underbrace{(\Lambda^{\frac{1}{2}}Y^\top)^{-1}U}_{B} \underbrace{U^\top \Lambda^{\frac{1}{2}}Y^\top}_{A} \boldX \\
    = & ~U (U^\top \Lambda^{\frac{1}{2}} Y^\top \boldX ) = \underbrace{U \Sigma V^\top}_{\mathrm{optimal~rank~Z~approximation}}.  
\end{align*}
\end{small}
%The last step is derived by noting that $U^\top Y^\top \Lambda^{\frac{1}{2}}\boldX = U^\top (U \Sigma V^\top + U' \Sigma' V'^\top) = \Sigma V^\top$ because $U$ and $U'$ are orthogonal.
\end{proof}


\tu{Weighted Linear Results:}
%We now describe an illustrative simulation to solve Prob. \ref{prob:codesign} using the SVD as in Theorem 2 for various scenarios $\lambda$.
For the weighted $\lambda > 0$ case, we solve Prob. \ref{prob:codesign} using the SVD as in Theorem 2. Fig. \ref{fig:LQR_simulation_3D} shows results for a toy linear problem with input and output dimensions $n=6$ and $m=3$, where we achieve optimal task performance with a $2\times$ compression gain. 
%Due to space constraints, we provide further details online \footnote{Our technical report \cite{tasknet} and Edge TPU software are available at \\ \url{https://sites.google.com/view/tasknet}.}. 
\revision{Our toy example shows that, even for linear systems, we achieve large compression gains by co-designing with a task objective, which mirror our subsequent results with complex DNNs.}
While we note our theory only applies to linear systems, such a theoretical underpinning is informative to understand our results for complex DNNs.

\input{figure_latex/D3_LQR.tex}


==> sections/sandeep_edits/abstract.tex <==
A variety of robots are increasingly using data-driven perception and planning models
that interface with classical model-based controllers. For example, drones can use computer vision models
to estimate target landing sites or navigation waypoints, which can be tracked by model predictive control (MPC). 
Often, such learned perception and planning models can be harmed by adversarial examples, which produce
erroneous state estimates or waypoints that ultimately lead to increased control costs. 
In contrast to prior work that synthesizes adversarial examples for single-step vision tasks, the key novelty of our work is to efficiently synthesize adversarial scenarios for multi-step, model-based control tasks. To do so, we leverage recently-developed differentiable MPC methods to calculate the sensitivity of a model-based controller to errors in state estimation, which in turn guides how we learn to synthesize adversarial visual scenarios. We illustrate that
\textit{re-training} vision models on these adversarial datasets improves robustness on out-of-distribution (OoD) test scenarios by up to \SC{28.2\%} compared to standard task-agnostic data augmentation. 
Our system is tested on examples of robotic navigation and
vision-based control of an autonomous air vehicle.
%on a photo-realistic autonomous aircraft simulation engine. 

%A variety of robots are increasingly using data-driven perception and planning models
%that interface with classical model-based controllers. For example, drones can use computer vision models
%to estimate target landing sites or navigation waypoints, which can be tracked by model predictive control (MPC). 
%Often, such learned perception and planning models can be harmed by adversarial examples, which produce
%erroneous state estimates or waypoints that lead to increased costs for an ultimate control task. 
%In this paper, we present a method to automatically synthesize adversarial visual scenarios
%for model-based control tasks. In contrast to prior work that synthesizes adversarial examples
%for single-step vision tasks, we calculate the sensitivity of a model-based controller to errors in state
%estimation, which guides efficient design of adversarial scenarios. We illustrate that fine-tuning
%learned vision and planning models on these adversarial datasets improves robustness on unseen test scenarios
%by up-to $X \times$, including on a photo-realistic autonomous aircraft simulator.


==> sections/sandeep_edits/backup/intro.tex <==
Imagine a drone that must safely land on diverse moving targets using its on-board camera and a learned perception module, such as a deep neural network (DNN). The drone's perception DNN, coupled with a downstream planning module, often outputs a sequence of waypoints that are tracked by MPC for a safe, low-cost trajectory \cite{borrelli2017predictive,Camacho2013}
. However, the drone will often operate in visual scenarios with radically different weather and terrain conditions than its original training distribution. In this paper, we ask whether we can automatically synthesize adversarial visual scenarios for multi-step, \textit{model-based} control tasks in order to re-train more robust robotic perception models.


Today's methods to train robust perception models include data augmentation \cite{albumentations,volpi2018generalizing}, domain randomization \cite{tobin2017domain,tobin2018domain}, and synthesis of adversarial examples for single-step vision tasks \cite{goodfellow2014explaining,hendrycks2021natural,xie2017adversarial}. 
Collectively, these methods would add synthetic visual examples by randomly cropping, rotating, or altering the hue of pixels in a training distribution or adversarially altering them to affect perceptual predictions. 
However, we observe that such augmentation methods are largely \textit{task-agnostic} and instead focus on improving vision models in isolation. As such, they often synthesize visual examples that might be ultimately benign for control, while missing those that directly affect key states.


Our work bridges recent advances in generative models \cite{Daniel_2021_CVPR,rybkin2021simple}, differentiable rendering \cite{park2019latentfusion,kato2020differentiable}, and differentiable MPC \cite{agrawal2020learningcontrol}. Collectively, these advances enable us to synthesize realistic visual scenes from a set of latent, often-interpretable, parameters and calculate their impact on control cost. Our principal contribution is a training procedure that efficiently perturbs the latent representation of a visual scene so that we render scenarios that are poor for control, but consistent with naturally-occurring data. Moreover, we can visualize
the latent representations of visual scenes to understand how task-driven, adversarial data augmentation improves the quality and diversity of training examples. Finally, we show that re-training perception models on such adversarial scenes improves their generalization on unseen examples compared to today's task-agnostic data augmentation methods.

\input{figures_latex/architecture_col}


%a highlight of 
%searching for adversarial visual scenes in the latent space of generated images is that we can visualize how adversarial data augmentation adds realistic test scenarios. 
%Crucially, we can also synthesize \textit{realistic} scenarios using \textbf{differentiable rendering} techniques, which map a set of latent parameters that describe a visual scene to a rendered visual input. Our principal contribution is a training procedure that perturbs the latent representation of a visual scene in order to synthesize adversarial, but plausible, visual examples that are poor for control. 

\textit{Literature Review: }
Our work is broadly related to adversarial reinforcement learning (RL) in robotics, data augmentation, differentiable model predictive control (MPC), and differentiable rendering methods. We now highlight how our approach differs from related work. 

It is well-known that many perception models are susceptible to adversarial examples \cite{goodfellow2014explaining,akhtar2018threat,hendrycks2021natural,xie2017adversarial}
. 
For example, techniques like the Fast Gradient Sign Method (FGSM) calculate the sensitivity of a pre-trained classifer to distortions in the image input, which guides how we synthesize small, human-imperceptible, pixel changes that cause  mis-classifications. However, to the best of our knowledge, there is very little work describing how such image perturbations ultimately affect \textit{multi-step, model-based} control tasks (e.g., navigation) that rely on state estimates from deep models.

%For example, techniques such as the Fast Gradient Sign method (among others) can create subtle, human-imperceptible pixel perturbations that produce wrong classifications from pre-trained vision models.
%These adversarial attacks, such as the popular Fast Gradient Sign Method (FGSM), essentially calculate the sensivity of a pre-trained classifer to distortions in the image input, which guides how we to make a bounded, adversarial perturbation to the original image. 




Our work is closest to, but distinct from, robust adversarial reinforcement learning (RARL) methods \cite{lutter2021robust,mandlekar2017adversarially,pinto2017robust,pan2019risk}. First, these methods aim to improve a \textit{control} policy, either 
by perturbing an agent's dynamics or introducing an adversarial RL agent that physically impedes progress. In stark contrast, we focus on fixed, model-based control policies (often represented by a convex program), and instead focus on re-training perception models that provide state estimates that serve as input parameters for convex MPC. To do so, we leverage recent advances in differentiable MPC
\cite{agrawal2020learningcontrol,agrawal2020learning,amos2018differentiable} to compute the sensitivity of the control cost to erroneous perceptual inputs. As such, we leverage the structure of the model-based controller to efficiently synthesize adversarial inputs as opposed to model-free RARL methods.

As noted earlier, today's standard data augmentation for computer vision \cite{volpi2018generalizing} is largely task-agnostic -- random image crops or rotations might change perception waypoints in a way that barely affects control cost.
Instead, our method leverages the structure of a model-based controller to targetedly perturb pixels that are most salient for control. The idea of task-driven data augmentation has already been applied to training graph neural networks (GNNs) by creating synthetic graphs with dropped nodes, edges etc. \cite{zakharov2019deceptionnet,chaitanya2019semi}. 
However, our key distinction is that we compute the sensitivity of a multi-step control task to pixel perturbations and innovate new loss functions that promote rendering of
realistic adversarial scenes. Finally, our work differs from gradient-free Bayesian Optimization \cite{abeysirigoonawardena2019generating} methods (e.g., for safety assurances for self-driving cars \cite{wang2021advsim,feng2021intelligent}) since we explicitly leverage the gradient of MPC's task cost.

\textit{Contributions:} Given prior work, our contributions are:  
\setlist{nolistsep}
\begin{enumerate}[noitemsep, leftmargin=*]
    \item We present a method to automatically synthesize adversarial examples for data-driven perception models that directly affect model-based control cost. 
    \item We develop a novel loss function that flexibly trades-off the realism of adversarial examples and their impact on control cost by learning perturbations in a latent space that generates visual scenes.
    \item We show that re-training on these synthesized examples leads to better performance on unseen test data than today's standard task-agnostic data augmentation. We demonstrate this result on examples of robotic navigation, arm manipulation and vision-based control of an aircraft.
\end{enumerate}

\textit{Paper Organization: } In Section \ref{sec:proposed_method}, we introduce how we integrate data-driven perception with differentiable MPC, and present our algorithm for adversarial scenario generation in Section \ref{sec:algorithm}. Then, in Section \ref{sec:experiments}, we show strong experimental performance for our algorithm on challenging OoD scenarios. Finally, we conclude in Section \ref{sec:conclusion}.


%1. First, we present a method to automatically synthesize adversarial examples for data-driven perception models that directly affect model-based control cost.
%
%2. Second, we develop a novel loss function that flexibly trades-off the realism of adversarial examples with their impact on control cost by learning perturbations in a latent space that generates visual scenes.
%%        %Specifically, we learn perturbations in a latent space that generates visual scenes and quantify that the rendered scenes are similar to original images, yet poor for control.
%
%3. We show that re-training on these synthesized examples leads to better performance on unseen test data than today's standard data augmentation. We demonstrate this result in a photo-realistic simulator where an aircraft must autonomously taxi using an on-board vision model \cite{XPlane,taxinetDataset}.
%\end{itemize}
%\SC{adversarial control RL: \cite{lutter2021robust} focuses on RL being more robust
%
%\cite{yang2021synthesis} focuses on safety specification violation
%
%differentiable MPC: \cite{agrawal2020learningcontrol,agrawal2020learning,amos2018differentiable}
%
%plain MPC: \cite{borrelli2017predictive,Camacho2013}
%
%data augmentation: \cite{volpi2018generalizing}
%
%AV space \cite{wang2021advsim}, uses Bayesian opt and LIDAR sensor failures. we look at diff MPC and gradient based approaches
%another AV: \cite{feng2021intelligent}
%
%Bayes Opt \cite{abeysirigoonawardena2019generating}
%
%CV standard adv examples: \cite{goodfellow2014explaining,akhtar2018threat,hendrycks2021natural,xie2017adversarial}
%
%domain randomization in robotics: \cite{tobin2017domain,tobin2018domain}
%
%task-driven data augmentation \cite{zakharov2019deceptionnet,chaitanya2019semi}
%
%X-Plane \cite{XPlane,taxinetDataset}
%
%}

==> sections/sandeep_edits/backup/method.tex <==
\subsection{Problem Statement}

% Fig 1: system diagram
% \input{figures_latex/architecture}

Fig. \ref{fig:expr_arch} shows a typical robotic learning system consisting of a \texttaskmodel \space and a \texttaskcost. In the case of self-driving cars, the \texttaskmodel \space consists of a perception module $\mpercep$ which takes sensory information of the scene, such as images or LiDAR, as inputs and derives a latent representation of the scene. The planning module $\mplan$ uses the latent representation to generate a safe and comfortable waypoint trajectory. The \texttaskcost \space is usually the motion planning cost. Thus, unsafe and aggressive waypoint trajectories are assigned higher costs, while safe and smooth trajectories are assigned lower costs. Next, we formally define the \texttaskmodel \space and the \texttaskcost.

\textit{Perception Model: }

\textit{Task Model:} The goal of the \texttaskmodel \space is to understand the robot's environment and generate future actions for the robot to achieve a specific task. We consider one of the most general \texttaskmodels, consisting of a perception module $\mpercep$ and a planning module $\mplan$. The perception module understands the environment around the robot by taking the sensory inputs from the environment. Specifically, the perception module $z = \mpercep (s)$  takes an image $s$ of the scene as input and outputs a latent representation $z$ of the scene. The planning module estimates the robot's current state and generates future actions for the robot. The planning module,$\mathbf{w}_F = \mplan(z, \mathbf{w}_P)$, takes the latent representation $z$ of the scene and a vector of the robot's past waypoints $\mathbf{w}_P$ as input and outputs a vector of future waypoints $\mathbf{w}_F$ for the robot to follow ($P$, $F$ is the number of waypoints). The waypoints $\mathbf{w}_P$ (or $\mathbf{w}_F$) are a sequence of $P$ (or $F$) tuples consisting of the robot's state. Robot's state is defined by the user for the specific use-case, for eg. $\mathbf{w}_P = \{ l_x, l_y, v, \theta \}_{i=1}^{P}$, where $l_x$ and $l_y$ are the robot's $x,y$ location in meters, $v$ is the speed in meters/sec and $\theta$ is robot's angle in radians. We will represent the whole \texttaskmodel, $\alltaskmodel$, by $\mtaskmodel$.

\textit{Task Cost:} To quantify the quality of the predicted waypoints by the \texttaskmodel, we use the \texttaskcost. The \texttaskcost, $\taskcost( \mathbf{w}_F ) \in \mathbb{R} $, measures the quality of $\mathbf{w}_F$ (the waypoints predicted by the \texttaskmodel) as a scalar value. For eg. the \texttaskcost \space could either measure smoothness of predicted waypoints $\mathbf{w}_F $, how much extra control will be utilized to execute waypoints $\mathbf{w}_F $ or check if the waypoints $\mathbf{w}_F$ violate the physical limits of the robot, etc. Therefore, undesired waypoints, $\mathbf{w}_F $, will have higher cost and vice versa. In this work, we will assume that $\taskcost$ is differentiable. 

%% The waypoints $\mathbf{w}_P$ ( or $\mathbf{w}_F$ ) are a sequence of P (or F) tuples consisting of $(x,y)$ locations of the robot, denoted by $\mathbf{w}_P = {(x_i, y_i)}_{i=0}^{P}$ (or F)
\textit{Differentiable Rendering Module:} \label{sec:diff_rendr_module}
In order to parametrize the input scenes, $s$, we introduce a differentiable rendering module $\render$. The differentiable rendering module, $ s = \render(\nu)$, generates the robot's scene input $s$ with the parameters $\nu$ and builds a latent space of the \texttaskmodel \space inputs, $s$, by parametrizing them with $\nu$. Therefore, the differentiable rendering module provides us with an ability to generate new scenes from the latent space. In our setting, $\render$ is a Decoder from a Variational Auto Encoder (CITE), described in section \ref{sec:expr_prelim}.

\textit{End-to-End Differentiable System:}
Using a differentiable \texttaskcost \space and a differentiable rendering module ($\render$) enables us to create an end-to-end differentiable mapping from input scene parameters, $\nu$, to the final \texttaskcost, as shown in Fig. \ref{fig:expr_arch}. This end-to-end differentiable mapping can be leveraged to back-propagate based on the final \texttaskcost \space w.r.t. to input scene parameters $\nu$. We use the differentiable rendering module to synthesize new scene inputs, $\bar{s}$, with a higher \texttaskcost \space compared to the original input scene $s$, we discuss this process in detail in section \ref{sec:method_setting} and Algorithm \ref{alg:train}.

\textit{The Problem:} A dataset, $\dataset$, containing $N$ tuples of inputs $x$ and ground-truth labels $y$ is denoted by $\datasetall$. For each $n \in N$, we have $x^{(n)} = \{s, \mathbf{w}_P\}$, the input scenes and past waypoints respectively. Similarly, we have $y^{(n)} = \{\mathbf{w}_F\}$ the future waypoints as labels. The dataset, $\dataset$, is separated into train dataset, $\datasettrain$ and a held-out test dataset, $\datasettest$. We train a \texttaskmodel \space on the train dataset, $\datasettrain$, to predict future waypoints, $\mathbf{w}_F$, given inputs $\{s, \mathbf{w}_P\}$. The \texttaskmodel \space trained on the dataset, $\datasettrain$, is represented as $\mtaskmodeldataset$. In a typical robot-learning system, we want the waypoints, $\mathbf{w}_F $ , predicted by $\mtaskmodeldataset$ to have lower \texttaskcost \space and also be robust to unseen scenarios, i.e. have good performance on the held-out dataset $\datasettest$. The problem we are tackling is what additional dataset $\datasetnewall$ with $M$ datapoints we can add to original dataset $\dataset$, such that a \texttaskmodel \space trained on combined dataset, $\dataset \cup \datasetnew$ will have a lower \texttaskcost \space and perform better on the held-out test dataset, $\datasettest$, compared to the original \texttaskmodel, $\mtaskmodeldataset$.  

% Specifically, each example $x = (s, \mathbf{w}_P)$ represents robot's image scene input $s$ and the history of waypoints $\mathbf{w}_P$. Using the inputs $x$, the \texttaskmodel \space predicts a ground-truth target vector $y = (\mathbf{w}_F)$ which represents the future waypoints for the robot to follow. 

% We experimentally show that a \texttaskmodel \mtaskmodel trained on the combined dataset \dataset $\cup$ \advdataset will have a lower average \texttaskcost \taskcost and will be more robust compared to a \texttaskmodel \mtaskmodel trained with standard single-level data augmentation techniques on out-of-distribution data. 

% Additionally, the new  \texttaskmodel \space will be more robust to out-of-distribution datapoints $ ( x^{'}, y^{'}) \notin$ \dataset $\cup$ \advdataset.

\subsection{Proposed Method} \label{sec:method_setting}
We hypothesize that we can significantly improve the task model if we re-train it on a dataset that includes scenarios where the original task model performs poorly. Thus, our goal is to synthetically generate adversarial scenarios for the original task model which lead to high task cost (i.e. poor performance). Our proposed method generates a new adversarial dataset $\advdatasetall$ from a given original dataset $\dataset$ such that the original \texttaskmodel \space $\mtaskmodeldataset$ will have a higher \texttaskcost \space $\taskcost( \hat{y} )$ for the new dataset $\advdataset$. 

To do so, we introduce the notion of a differentiable adversary to generate the new dataset $\advdataset$, shown in orange in Fig. \ref{fig:expr_arch}. 
Specifically, the adversary maps the original latent scene representation $\nu$ to a perturbed represenation $\bar{\nu} = \adv(\nu; \advparam)$, where $\advparam$ are trainable parameters. Our goal is to train the parameters such that the adversarial scene representation $\bar{\nu}$ increases the task cost $\taskcost$ compared to the original scene representation $\nu$. 

\textit{Adversary Loss Function:} 
We now introduce a novel loss function to train the adversary $\adv$. 
Intuitively, the adversary's loss function must perturb the latent scene representation $\nu$ to $\bar{\nu}$ such that the \texttaskcost \space increases. At the same time, it must ensure that the new rendered scene from $\bar{\nu}$ is realistic and fairly close to $\nu$. This is necessary since we want to augment our training dataset with scenes represented by $\bar{\nu}$ that a robot can plausibly encounter during real-world test deployment.
Therefore, the following adversarial loss function must delicately balance the differentiable \texttaskcost \space and distance loss between $\bar{\nu}$ and $\nu$. 

\textit{Adversarial Task Cost: }
Given an original latent representation $\nu$ of the scene, we invoke the adversary
to generate the adversarial latent representation by $\bar{\nu} = \adv(\nu; \advparam) $. 
Then, we simply invoke the end-to-end differentiable modules in Fig. 1. Namely, the renderer first generates a new perturbed visual scene $\bar{s} = \render(\bar{\nu})$. Next, given this adversarial scene $\bar{s}$, the task model outputs a new waypoint prediction $\mathbf{w}_F = \mplan(\bar{s}, \mathbf{w}_P)$.  Finally, we calculate the new \texttaskcost \space $ \taskcost(\mathbf{w}_F)$.

\textit{Consistency (Distance) Loss: }
%We must be careful to generate realistic, but adversarial, scenarios that can possibly occur during real-world robotic deployment. 
%Otherwise, generating unrealistic, and possibly over-adversarial, scenarios might not help in improving the \texttaskmodel's robustness on real OoD data. 
Generating unrealistic, and possibly over-adversarial, scenarios might not help in improving the \texttaskmodel's robustness on real OoD data. 
To incentivize realism, we introduce a consistency loss $\distloss \in \mathbb{R}$. The consistency loss measures the distance between the original input $s$ and the adversarially generated scene $\bar{s}$ in the latent space of
$\render$. Calculating the distance loss in the \textit{latent space} is a novelty of our loss function based on the observation that similar scenes $s$ and $\bar{s}$ might be very far in the high-dimensional image space but might be close in the latent space of the renderer $\render$. Moreover, if the latent space parameters $\nu$ have \textit{physical meaning}, such as the mass, positions, and colors of key objects in the scene, we can interpret the distance in the $\nu$
space. In our experiments, we use the $L_2$ norm distance between latent space variables $\bar{\nu}$ and $\nu$, although our general method can accomodate other differentiable distance loss functions. 

%Specifically, we calculate the distance loss $\distloss$ between latent space variables $\nu$ and $\bar{\nu}$, instead of the actual scene $s$ and $\bar{s}$. The distance loss $\mathcal{I}$ is weighted by $\kappa$ in the optimization step, which controls how much we allow $\bar{s}$ to deviate from $s$. We use the L2-norm for the distance loss, actual implementation is discussed in section \ref{sec:expr_prelim}.

\textit{Overall Adversarial Loss Function: }
Finally, our adversarial loss function allows us to trade-off extra control cost while incentivizing realism of the rendered synthetic scene:   
\begin{equation} \label{eq:adv_loss}
\begin{aligned}
  \loss = \hat{J}( \bar{\nu}, \advparam )  \mathbf{-} \kappa \distloss. 
  % \max_{\advparam} L ( \bar{\nu}, \advparam ) = \hat{J}( \bar{\nu}, \advparam )  \mathbf{-} \kappa \distloss \mathbf{-} \lambda ||\advparam||_{p} 
\end{aligned}
\end{equation}

Here, the distance loss is weighted by $\kappa$ in the loss function, which can be flexibly set by a roboticist depending on how adversarial they prefer rendered scenarios to be.  

\textit{Adversary Training:} Algorithm \ref{alg:train} shows \SC{our} complete adversarial training procedure. We iterate over each point in the training dataset and generate that point's corresponding adversarial example by performing gradient descent on our weighted loss function that trades-off increased control cost with a consistency loss. Then, we save the most adversarial synthetic examples generated by trainable adversary $\adv$ for subsequent data augmentation. To do so, we decided to use a new adversary for each datapoint rather than training a common adversary for the whole dataset. 

Starting from line \ref{ln:for1_loop}, we iterate through the original dataset $\dataset$. Each datapoint $x_{i}$ is a tuple of input scene $s_i$ and past waypoints  $\mathbf{w}_P$.
Lines \ref{ln:init_nu}-\ref{ln:init_tuple} describe how we initialize a \textit{new trainable} adversary for each datapoint.
First, we obtain the latent space representation $\nu_i$ of the datapoint $x_i$ from the differentiable renderer $\render$ in line \ref{ln:init_nu}. In line \ref{ln:init_adv}, we initialize a new adversary $\adv$ with random weights $\advparam_{k=0}$, which will be specific to the datapoint $x_i$. Since we train the adversary parameters for $K$ gradient descent steps, we use subscript $k$ to indicate the adversary's parameters at training step $k$.
Likewise, we index the new adversarially-generated latent representation at each step $k$ by $\bar{\nu}_k$.  Henceforth, the notation $\bar{x}$ indicates the perturbed (adversarial) version of variable $x$, such as a new adversarial data-point. Finally, in lines \ref{ln:init_adv_nu}-\ref{ln:init_tuple}, we initialize 
a tuple $(\bar{x}, \bar{y}, \bar{\nu})$ that will indicate the adversarially generated datapoint, label, and latent representation. They are initialized to the \textit{original} training dataset's values and will be adversarially perturbed next.
%in the next part of the algorithm.

The crux of our algorithm is in lines \ref{ln:for2_loop}-\ref{ln:for2_end}, where we perform $K$ gradient update steps to train the adversary $\adv$. In each gradient step $k$, we update the adversary parameters to $\advparam_{k}$ using adversarial loss function $ L(\nu, \bar{\nu}_{k}; \advparam_{k-1} ) $ and back-propagation (lines \ref{ln:calc_nuk}-\ref{ln:calc_grad}). In lines 15-19, we store the adversarial tuple $( \bar{x}_k , y_i, \bar{\nu_{k}} ) $ if it has higher task cost $\hat{J}( \mathbf{w}_F )$ than the previous best
\texttaskcost \space $J^{\star}$. Finally, after $K$ gradient steps, we append the best adversarial datapoint $ (\bar{x}, \bar{y}, \bar{\nu}) $ to dataset $\advdataset$ in line \ref{ln:append_data}. Crucially, we keep all the network weights frozen during adversarial training, and only adversary parameters $\advparam$ are updated. At the end, we have generated a new adversarial dataset for data augmentation.

\begin{small}
\begin{algorithm}[t]
\DontPrintSemicolon
\SetNoFillComment % <---------------------------
\SetAlgoLined
    Initialize \SC{empty} new adversarial dataset $\advdataset$ = \{\}  \;  \label{ln:init_adv_dataset}
\For{$ (x_i = \{s_i, \mathbf{w}_P  \}, y_i) \gets$  $\datasetall$,  $0 \leq i \leq N$ \label{ln:for1_loop}}  {
    % $x_i = \{s_i, \mathbf{w}_P  \}$ \; \label{ln:init_data} 
    Get $s_i$'s differentiable renderer params $\nu_i$ \; \label{ln:init_nu} 
    Init. adver $\adv( \nu_i ; \advparam_{k=0} ) $ with random $\advparam_{k=0}$   \; \label{ln:init_adv} 
    \SC{Init. \textit{adversarial} latent rep.} $\bar{\nu}_{k =0 } = \nu_i $ \; \label{ln:init_adv_nu} 
    Best Task Loss $ J^{\star}  = - \infty $ \; \label{ln:init_j} 
    \SC{Init. Adv. Tuple $(\bar{x}, \bar{y}, \bar{\nu}) = (x_i, y_i, v_i)$} \; \label{ln:init_tuple} 
    \For{$k~ \gets 1 $ \KwTo K \label{ln:for2_loop}}{ 
    Get adv. latent params $ \bar{\nu}_{k} = \adv(  \bar{\nu}_{k - 1}  ; \advparam_{k-1} )  $ \; \label{ln:calc_nuk} 
    Render perturbed scene $\bar{s}_{k} = \render(\bar{\nu}_{k}) $ \; \label{ln:calc_sk} 
    Get planner waypoints $\mathbf{w}_F = \mtaskmodel(\bar{s}_{k}, \mathbf{w}_P)$ \; \label{ln:calc_wf} 
    Calculate \texttaskcost \space $J( \mathbf{w}_F )$ \; \label{ln:calc_J} 
    Calculate Loss $L(\nu_i, \bar{\nu}_{k}; \advparam_{k-1} ) $  \; \label{ln:calc_loss} 
    $\advparam_{k} \gets \textsc{BackProp}(\advparam_{k-1}, L(\nu_i, \bar{\nu}_{k};  \advparam_{k-1}))$ \; \label{ln:calc_grad} 

    \If{ $J( \bar{\nu_{k}},  \advparam_{k-1} ) \geq J^{\star}$  \label{ln:update_if}  } {
        Update most adv. scene $\bar{x}_k = \{\bar{s}_{k}, \mathbf{w}_P  \} $ \; \label{ln:update_xk}
        $ (\bar{x}, \bar{y}, \bar{\nu}) = ( \bar{x}_k , y_i, \bar{\nu_{k}} ) $  \; \label{ln:update_tuple}
        $ J^{\star} \gets J $ \; \label{ln:update_J}
    } \label{ln:for2_end}
    } \label{ln:for1_end}
    Append $ (\bar{x}, \bar{y}, \bar{\nu}) $ to  $\advdataset$ \; \label{ln:append_data}
 } \caption{\textbf{Adversary Training}}
 \label{alg:train}
\end{algorithm}
\end{small}

We now experimentally show that a \texttaskmodel \space $\mtaskmodel$ trained on the combined dataset $\dataset$ $\cup$ $\advdataset$ will have a lower average \texttaskcost \space $\taskcost$ and will be more robust compared to a \texttaskmodel \space $\mtaskmodel$ trained with standard single-level data augmentation techniques on out-of-distribution (OoD) data. 



==> sections/sandeep_edits/backup/preamble.tex <==
\newtheorem{problem}{Problem}

\newcommand{\render}{\psi_{\mathrm{render}}}
\newcommand{\adv}{f_{\mathrm{adv}}}
\newcommand{\distloss}{\mathrm{I}(\nu, \bar{\nu})}

\newcommand{\dataset}{\mathcal{D}}
\newcommand{\datasetnew}{\mathcal{D}_{\mathrm{new}}}
\newcommand{\advdataset}{\mathcal{D}_{\mathrm{adv}}}

\newcommand{\datasetall}{\dataset = \{x, y\}_{i=1}^{N}}
\newcommand{\datasetnewall}{\datasetnew = \{x, y\}_{i=1}^{M}}
\newcommand{\advdatasetall}{\advdataset = \{x, y\}_{i=1}^{N}}

% Orig
\newcommand{\datasettrain}{\dataset^{\mathrm{train}}}
\newcommand{\datasettest}{\dataset^{\mathrm{test}}}

% Orig
\newcommand{\datasetorigtrain}{\dataset_{\mathrm{orig}}^{\mathrm{train}}}
\newcommand{\datasetorigtest}{\dataset_{\mathrm{orig}}^{\mathrm{test}}}

% Add
\newcommand{\datasetaddtrain}{ \mathcal{D}_{\mathrm{add}}^{\mathrm{train}} }
\newcommand{\datasetaddtest}{ \mathcal{D}_{\mathrm{add}}^{\mathrm{test}}}

% Aug
\newcommand{\datasetaugtrain}{ \mathcal{D}_{\mathrm{aug}}^{\mathrm{train}} }
\newcommand{\datasetaugtest}{ \mathcal{D}_{\mathrm{aug}}^{\mathrm{test}}}

% Adver
\newcommand{\datasetadvtrain}{ \advdataset^{\mathrm{train}} }
\newcommand{\datasetadvtest}{ \advdataset^{\mathrm{test}}}

% afternoon
\newcommand{\datasetafternoon}{ \mathcal{D}_{\mathrm{afternoon}} }
\newcommand{\datasetafternoontrain}{ \datasetafternoon^{\mathrm{train}} }
\newcommand{\datasetafternoontest}{ \datasetafternoon^{\mathrm{test}}}

% morning
\newcommand{\datasetmorning}{ \mathcal{D}_{\mathrm{morning}} }
\newcommand{\datasetmorningtrain}{ \datasetmorning^{\mathrm{train}} }
\newcommand{\datasetmorningtest}{ \datasetmorning^{\mathrm{test}}}

% overcast
\newcommand{\datasetovercast}{ \mathcal{D}_{\mathrm{overcast}} }
\newcommand{\datasetovercasttrain}{ \datasetovercast^{\mathrm{train}} }
\newcommand{\datasetovercasttest}{ \datasetovercast^{\mathrm{test}}}

% night
\newcommand{\datasetnight}{ \mathcal{D}_{\mathrm{night}} }
\newcommand{\datasetnighttrain}{ \datasetnight^{\mathrm{train}} }
\newcommand{\datasetnighttest}{ \datasetnight^{\mathrm{test}}}

\newcommand{\datasetood}{ \mathcal{D}_{\mathrm{OoD}} }
\newcommand{\datasetoodtest}{ \datasetood^{\mathrm{test}}}

\newcommand{\mpercep}{\phi_{\mathrm{perception}}}
\newcommand{\mplan}{\phi_{\mathrm{plan}}}
% \newcommand{\taskcost}{\hat{J}_{\mathrm{MPC}}}
\newcommand{\taskcost}{J}
\newcommand{\mtaskmodel}{\phi_{\mathrm{task\_model}}}
\newcommand{\mtaskmodeldataset}{\phi_{\mathrm{task\_model}}^{\dataset}}
\newcommand{\alltaskmodel}{\mathbf{w}_F = \mtaskmodel(s, \mathbf{w}_P)}

% \newcommand{\texttaskmodel}{\textsc{Task Model}}
% \newcommand{\texttaskcost}{\textsc{Task Cost}}
\newcommand{\texttaskmodel}{task model}
\newcommand{\texttaskcost}{task cost}
\newcommand{\texttaskmodels}{task models}
\newcommand{\texttaskcostss}{task costs}

\newcommand{\mpccontrol}{\hat{u}}
\newcommand{\mpcstate}{\hat{x}}
\newcommand{\advparam}{\theta^{\mathrm{adv}}}

\newcommand{\loss}{L\left( \nu, \bar{\nu}, \advparam \right)}


==> sections/sandeep_edits/backup/problem_formulation.tex <==
\textit{Differentiable Perception Module: } The robot's differentiable perception module $\mpercep$ maps a high-dimensional visual observation $s$ into a low-dimensional scene embedding $z$, denoted by: 
\begin{eqnarray*}
    z = \mpercep(s; \percepparam). 
\end{eqnarray*}
Here, $\percepparam$ are parameters of the perception module, such as a DNN. Next, the robot must use the scene embedding $z$ to plan a safe, collision-free trajectory to achieve its task. Often, we can represent a robot's desired trajectory by a sequence of waypoints or desired configurations a robot should follow. For example, for a 2-d planar robot, a waypoint could be a sequence of landmark poses in the $x-y$ plane to move along. Concretely, the differentiable planning module maps scene
embedding $z$ and a vector of $P$ past waypoints $w_p$ to a vector of $F$ future waypoints to follow, denoted by: 
\begin{eqnarray*}
    w_F = \mplan(z; \planparam). 
\end{eqnarray*}
Here, $\planparam$ are parameters of the differentiable planner. 

\textit{Differentiable MPC: } The next step is to control the robot to follow the waypoints $w_F$ with minimal control cost. Suppose the robot is at some initial state $\zeta_t$ and has a planning horizon of $F$ steps. Then, its controller $\pi$ should map the initial state $\zeta_t$ and future waypoints $w_F$ into a sequence of controls from $t$ to $t+F$, denoted by 
$u_{t:t+H} = \pi(\zeta_t, w_F; \MPCparam)$. Here, $\MPCparam$ could represent feedback gains for MPC. Crucially, we define a task (control) cost $J(w_F; \percepparam, \planparam, \MPCparam)$ which depends on the final waypoints the robot tracks $w_F$. Since the waypoints $w_F$ depend on the previous perception and planning modules, the cost $J$ implicitly depends on their parameters too. 

%\textit{How does the end-to-end differentiable pipeline perform under adversarial visual inputs?}
\textit{Differentiable Rendering Module:} \label{sec:diff_rendr_module}
In this paper, we analyze how the ultimate task (control) cost $J$ would increase if the robot observes an adversarial visual input $\bar{s}$ instead of original image $s$. To do so, we need a process to generate, or render, realistic adversarial scenes $\bar{s}$. Fortunately, recent progress in generative models and differentiable rendering techniques in computer graphics makes rendering scenes $\bar{s}$ possible. A differentiable renderer $s = \render(\nu; \renderparam)$ generates the robot's
scene $s$ from latent parameters $\nu$ that describe the scene and internal parameters $\renderparam$ of the rendering model. Often, the latent representation $\nu$ of scene $s$ could be interpretable and controllable, such as the mass, pose, lighting, and texture of different objects. Crucially, the rendering module empowers us to generate new scenes, including adversarial ones $\bar{s}$, from the latent space of $\nu$ parameters. Without loss of generality, the renderer in our pipeline could also be a conventional generative model, such as the decoder in a Varational Autoencoder (VAE) or a Generative Adversarial Network (GAN).
All we require is a differentiable mapping from scene parameters $\nu$ to images $s$. Henceforth, we use the term differentiable renderer for $\render$, even though we use VAE decoders since our work uses custom datasets without differentiable rendering pipelines. 

\textit{End-to-End Differentiable System:}
This paper considers how we can efficiently perturb the latent representation of an original image $\nu$ to a new representation $\bar{\nu}$ (and rendered scene $\bar{s}$) that increases MPC task cost. Since every block we described in Fig. \ref{fig:expr_arch} is differentiable, we 
we have an end-to-end differentiable mapping from scene parameters $\nu$ to ultimate task cost $J$. As such, we back-propagate the gradient of the MPC task cost $J$ with respect to scene parameters $\nu$ to efficiently search for adversarial scene parameters $\bar{nu}$, which is the crux of our method. 

\textit{Training and Test Datasets: }
We first formalize our dataset notation before formally defining our problem statement.
A dataset contains $N$ tuples of inputs $x$ and ground-truth labels $y$ denoted by $\datasetall$. Specifically, each example $x = (s, \nu, \mathbf{w}_P)$ represents the robot's scene input $s$, corresponding latent renderer representation $\nu$,  and waypoint history $\mathbf{w}_P$. From these, the task model predicts a ground-truth target vector $y = (\mathbf{w}_F)$ of future robot waypoints. In practice, these labels can come from an oracle planner to emulate, such as a Frenet Planner, that has perfect access to ground-truth scenes $s$ and waypoints $w_p, w_F$. Henceforth, the subscript $b$ in the dataset notation $\dataset^a_b$ will represent the type of dataset, such as whether it is an original image, from data augmentation, or adversarial training. 
Likewise, the superscript $a$ will represent if the dataset is from the \textit{train} or \textit{test} distribution. For example, the original training and test datasets are given by $\datasetorigtrain$ and $\datasetorigtest$. Likewise, a held-out OoD test dataset is denoted by $\datasetOoDtest$. Crucially, we define a training function $\textsc{Train}$ that uses supervised learning to train the task model to output correct waypoints $w_F$ (label $y$) given the scene $s$ (part of input $x$). For
example, the notation $\percepparam^0, \planparam^0 \gets \textsc{Train}(\datasetorigtrain)$ indicates we train the nominal task model parameters on the original training dataset.

\textit{Problem Statement: } For a focused contribution, we consider a practical scenario where the robot has an MPC controller with fixed parameters $\MPCparam$. Moreover, given a dataset of original training images and waypoints $\datasetorigtrain$, we have already pre-trained a nominal task model $\percepparam^0, \planparam^0$. Given these inputs, 
our problem is generate an additional dataset $\datasetnewall$ of $M$ datapoints such that re-training the perception and planning models on combined dataset $\dataset \cup \datasetnew$ will minimize task cost $J$ on a held-out OoD test dataset $\datasettest$. We only consider $M$ added examples to limit the training costs. Formally, our problem becomes: 

\begin{eqnarray*}
    & \mathrm{Find~new~dataset~} \datasetnew \mathrm{~such~that} \\
    & \min_{\percepparam', \planparam'} \mathbb{E}_{(\nu', s', w_F) \sim \datasettest} J(\nu'; \percepparam', \planparam', \MPCparam) \\
    & \mathrm{where} \\
    & \planparam', \percepparam' \gets \textsc{Train}(\dataset \cup \datasetnew)
\end{eqnarray*}

In general, it is hard to analytically find the ``best'' additional dataset of $M$ points to minimize task cost on OoD data. This is because (a) the re-trained perception and planning model parameters $\planparam'$ and $\percepparam'$ result from training a non-convex DNN and (b) the test dataset $\datasettest$ is a-priori unknown. We now describe our hypothesis that adversarially generated scene parameters for the MPC \textit{control} task will lead to the better generalization on OoD data.  


%\textit{The Problem:} 
%A dataset, $\dataset$, containing $N$ tuples of inputs $x$ and ground-truth labels $y$ is denoted by $\datasetall$. For each $n \in N$, we have $x^{(n)} = \{s, \mathbf{w}_P\}$, the input scenes and past waypoints respectively. Similarly, we have $y^{(n)} = \{\mathbf{w}_F\}$ the future waypoints as labels. The dataset, $\dataset$, is separated into train dataset, $\datasettrain$ and a held-out test dataset, $\datasettest$. We train a \texttaskmodel \space on the train dataset, $\datasettrain$, to predict future waypoints, $\mathbf{w}_F$, given inputs $\{s, \mathbf{w}_P\}$. The \texttaskmodel \space trained on the dataset, $\datasettrain$, is represented as $\mtaskmodeldataset$. 
%In a typical robot-learning system, we want the waypoints, $\mathbf{w}_F $ , predicted by $\mtaskmodeldataset$ to have lower \texttaskcost \space and also be robust to unseen scenarios, i.e. have good performance on the held-out dataset $\datasettest$. 

%The problem we are tackling is what additional dataset $\datasetnewall$ with $M$ datapoints we can add to original dataset $\dataset$, such that a \texttaskmodel \space trained on combined dataset, $\dataset \cup \datasetnew$ will have a lower \texttaskcost \space and perform better on the held-out test dataset, $\datasettest$, compared to the original \texttaskmodel, $\mtaskmodeldataset$.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% OLD NOTES HERE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%4. motivate that this in a fast emerging trend (cite differentiable physics renderers, graphics pipelines)
%5. then describe renderer that renders scene in simulation, has a continous space of latent  parameters
%6. ask if we can perturb the parameters in latent space to generate new images bar s that increase task cost

%\textit{Differentiable Rendering Module:} \label{sec:diff_rendr_module}
%In order to parametrize the input scenes, $s$, we introduce a differentiable rendering module $\render$. The differentiable rendering module, $ s = \render(\nu)$, generates the robot's scene input $s$ with the parameters $\nu$ and builds a latent space of the \texttaskmodel \space inputs, $s$, by parametrizing them with $\nu$. 
%Therefore, the differentiable rendering module provides us with an ability to generate new scenes from the latent space. 
%In our setting, $\render$ is a Decoder from a Variational Auto Encoder (CITE), described in section \ref{sec:expr_prelim}.
%

%We hypothesize that we must first synthesize adversarial images $\bar{s}$ from which the robot achieves the worst control cost. Then, we further hypothesize that adding synthetic adversarial images $\bar{s}$ to the original training dataset of images $s$, will allow us to re-train a perception and planning model that perform robustly
%For a focused contribution, we consider a practical scenario where the robot has a model-based, differentiable controller with fixed parameters $\MPCparam$. Moreover, we have a training distribution of images $D_{\mathrm{train}}$ where original images $s$ are drawn from, denoted by $s \sim D_{\mathrm{train}}$. From this distribution, we pre-train nominal parameters for the perception and planning modules, denoted by $\perceptionparam^0, \planparam^0$. 

%\edits{add more here ...}
%The key question we consider is how the original perception and planning modules would fare
%1. ask how the pre-trained perception modules would fare under test distro?
%2. then, say if we can synthesize adversarial scenarios and add them to our training distro, would we do better on test dataset
%
%3. to do so, we need a process to generate (or render) adversarial images
%4. motivate that this in a fast emerging trend (cite differentiable physics renderers, graphics pipelines)
%5. then describe renderer that renders scene in simulation, has a continous space of latent  parameters
%6. ask if we can perturb the parameters in latent space to generate new images bar s that increase task cost

%\textit{Differentiable Rendering Module:} \label{sec:diff_rendr_module}
%In order to parametrize the input scenes, $s$, we introduce a differentiable rendering module $\render$. The differentiable rendering module, $ s = \render(\nu)$, generates the robot's scene input $s$ with the parameters $\nu$ and builds a latent space of the \texttaskmodel \space inputs, $s$, by parametrizing them with $\nu$. Therefore, the differentiable rendering module provides us with an ability to generate new scenes from the latent space. In our setting, $\render$ is a Decoder from a Variational Auto Encoder (CITE), described in section \ref{sec:expr_prelim}.

%\textit{End-to-End Differentiable System:}
%Using a differentiable \texttaskcost \space and a differentiable rendering module ($\render$) enables us to create an end-to-end differentiable mapping from input scene parameters, $\nu$, to the final \texttaskcost, as shown in Fig. \ref{fig:expr_arch}. This end-to-end differentiable mapping can be leveraged to back-propagate based on the final \texttaskcost \space w.r.t. to input scene parameters $\nu$. We use the differentiable rendering module to synthesize new scene inputs, $\bar{s}$, with a higher \texttaskcost \space compared to the original input scene $s$, we discuss this process in detail in section \ref{sec:method_setting} and Algorithm \ref{alg:train}.
%
%\textit{The Problem:} A dataset, $\dataset$, containing $N$ tuples of inputs $x$ and ground-truth labels $y$ is denoted by $\datasetall$. For each $n \in N$, we have $x^{(n)} = \{s, \mathbf{w}_P\}$, the input scenes and past waypoints respectively. Similarly, we have $y^{(n)} = \{\mathbf{w}_F\}$ the future waypoints as labels. The dataset, $\dataset$, is separated into train dataset, $\datasettrain$ and a held-out test dataset, $\datasettest$. We train a \texttaskmodel \space on the train dataset, $\datasettrain$, to predict future waypoints, $\mathbf{w}_F$, given inputs $\{s, \mathbf{w}_P\}$. The \texttaskmodel \space trained on the dataset, $\datasettrain$, is represented as $\mtaskmodeldataset$. In a typical robot-learning system, we want the waypoints, $\mathbf{w}_F $ , predicted by $\mtaskmodeldataset$ to have lower \texttaskcost \space and also be robust to unseen scenarios, i.e. have good performance on the held-out dataset $\datasettest$. The problem we are tackling is what additional dataset $\datasetnewall$ with $M$ datapoints we can add to original dataset $\dataset$, such that a \texttaskmodel \space trained on combined dataset, $\dataset \cup \datasetnew$ will have a lower \texttaskcost \space and perform better on the held-out test dataset, $\datasettest$, compared to the original \texttaskmodel, $\mtaskmodeldataset$.  
% Specifically, each example $x = (s, \mathbf{w}_P)$ represents robot's image scene input $s$ and the history of waypoints $\mathbf{w}_P$. Using the inputs $x$, the \texttaskmodel \space predicts a ground-truth target vector $y = (\mathbf{w}_F)$ which represents the future waypoints for the robot to follow. 
% We experimentally show that a \texttaskmodel \mtaskmodel trained on the combined dataset \dataset $\cup$ \advdataset will have a lower average \texttaskcost \taskcost and will be more robust compared to a \texttaskmodel \mtaskmodel trained with standard single-level data augmentation techniques on out-of-distribution data. 
% Additionally, the new  \texttaskmodel \space will be more robust to out-of-distribution datapoints $ ( x^{'}, y^{'}) \notin$ \dataset $\cup$ \advdataset.


==> sections/sandeep_edits/experiments.tex <==
We now evaluate \SC{our method (Algorithm \ref{alg:train})} on two diverse tasks. 
\SC{The first task is a simple, but illustrative, toy example of robotic motion planning.} In the second experiment, an \SC{autonomous aircraft must taxi} by tracking a runway center-line based on visual inputs in challenging weather conditions. 
%\SC{that are rendered} in a photo-realistic simulator.

\subsection{Experiment Preliminaries} \label{sec:expr_prelim}

\textit{Adversary Model:} We use a linear model for our adversary $\adv( \nu ; \advparam ) = \advparam \nu$, where $\advparam \in \mathbb{R}^{n \times n }$.
\SC{Our subsequent experiments show that a linear adversary is expressive enough to generate realistic scenarios that are poor for control tasks. Our method allows for more complex neural network adversary models since it is fully differentiable.}
    
\textit{Distance Loss and Regularization:} We \SC{use} the \SC{mean squared error (MSE)} as the consistency loss $\distloss = \left|\left| \nu - \bar{\nu} \right|\right|_{2} ^{2}$ in Eq. \eqref{eq:adv_loss}. This ensures that the adversarial scene's latent representation does not deviate too far from that of the original.
\SC{Since the full pipeline in Fig. \ref{fig:expr_arch} is differentiable, we can easily train the adversary by computing the gradient of the loss $L$ with respect to the adversary's parameters $\advparam$ using automatic differentiation libraries. Finally, as shown in the experiments, the consistency loss weight $\kappa$ can be flexibly set by the user based on how adversarial they want synthetic examples to be.}

\textit{Variational Autoencoder (VAE):} We use a VAE \cite{kingma2014autoencoding} as the differentiable rendering module $\render$ \SC{from Section \ref{sec:diff_rendr_module}}. \SC{VAEs} have gained significant popularity because of their \SC{more stable training procedures compared to Generative Adversarial Networks (GANs)}. 
%Additionally, VAEs encode data input \SC{$s$} in a lower-dimensional subspace (the latent space) from the original higher-dimensional space. 
It is
important to note that we only use the VAE \textit{Decoder} as the differentiable rendering module, which takes parameters $\nu$ as input and outputs the image $s$ of the scene. We keep the \textit{Decoder} frozen after training it initially on the \SC{whole training} dataset.

\textit{Differentiable Model Predictive Control (MPC):} In both the tasks, we will formulate the \texttaskcost \space $\taskcost(w_F)$ \SC{for an} MPC problem with quadratic costs and linear constraints, as shown in Eq. \ref{eq:track_mpc}. The planning module provides the MPC controller with \SC{a} waypoint vector  $w_F$ for $F$ future timesteps to track. 
The robot's state at discrete time $t$ is denoted by $\mpcstate_t \in \mathbb{R}^{4 \times 1}$, defined as $\mpcstate_t = \{l_x, l_y, v, \theta \}$ for both experiments. Here, $l_x$ and $l_y$ are the robot's $x,y$ location in meters, $v$ is the speed in meters/sec, and $\theta$ is the robot's heading angle in radians. The robot's control input at time $t$ is defined as $\mpccontrol_t = \{a, \gamma \}$, where $a$ is \SC{the} robot's acceleration in $m/s^2$ and $\gamma$ is \SC{the} robot's steering input in radians/sec. 

\SC{Our main goal is to formulate the task cost $\taskcost(w_F)$, which is a standard quadratic cost penalizing state deviations and control effort. Namely, $\mathbf{Q} \in \mathbb{R}^{4 \times 4} $ is the state cost matrix and $\mathbf{R} \in \mathbb{R}^{2 \times 2} $ is the control cost matrix.} The matrices $\mathbf{A} \in \mathbb{R}^{4 \times 4} $ and $\mathbf{B} \in \mathbb{R}^{4 \times 2} $ define the robot's dynamics. For the first experiment, we use standard double integrator
dynamics while the second experiment uses linearized unicycle dynamics. The robot has box control constraints $u_{min} \leq \mpccontrol_t \leq u_{max}$ bounding the minimum and maximum acceleration and steering angle. Likewise, box state constraints $ \mpcstate_{min} \leq \mpcstate_t \leq \mpcstate_{max}$ define limits on the velocity and linear obstacle avoidance constraints. These constraints, used only in our first motion planning example, were calculated by drawing perpendicular hyperplanes from the
obstacles. Given a set of $F$ future waypoints $w_F = \{w_0, w_1, \ldots, w_{F-1}\}$ for a planning horizon starting at $t=0$, our MPC task cost and problem become:  
    \begin{equation} \label{eq:track_mpc}
        \begin{aligned}
            \min_{\mpcstate_{0:F}, u_{0:F-1}} ~J(w_F)  &=\sum_{t=0}^{F} (w_{t}^{\top} - \mpcstate_t^{\top} ) \mathbf{Q} (w_{t} -\mpcstate_t) +\sum_{t=0}^{F-1} \mpccontrol_t^{\top} \mathbf{R} \mpccontrol_t \\
    \text {such that~~} & \mpcstate_{t+1} =\mathbf{A}\mpcstate_t + \mathbf{B} \mpccontrol_t \\
    & u_{min} \leq \mpccontrol_t \leq u_{max}  \\
    & \mpcstate_{min} \leq \mpcstate_t \leq \mpcstate_{max}.  \\
        \end{aligned}
    \end{equation}

Our key step is to calculate the sensitivity of the task cost $J$ to adversarial perturbations in the image $s$ in order to train the adversary. To do so, we use advances in differentiable MPC to calculate the gradient of MPC's solution and task cost (a convex program) with respect to its problem parameters (i.e., waypoint predictions $w_F$). Then, we back-propagate through the differentiable pipeline in Fig. \ref{fig:expr_arch} to compute the gradient of MPC's task
cost with respect to
the adversary's parameters. Both experiments use the \textsc{cvxpylayers} Pytorch library
for differentiable convex programs \cite{cvxpylayers2019}.
    
\textit{Architectures:} Both experiments use DNNs for all modules in Fig. \ref{fig:expr_arch} except model-based control. The perception module $\mpercep$ is a convolutional VAE \textit{Encoder} since it must map image $s$ to an embedding $z$  that can be used by the planner. For the planner, we achieved success with both simple multi-layer perceptrons (MLPs) and CNNs.  
%The type of deep network in the \texttaskmodel \space is not essential for 
Our algorithm is agnostic to the type of deep network since it aims to improve any general, differentiable \texttaskmodel. Further details about model and training parameters are provided in Appendix \ref{sec:experiment_details}.

%In both the tasks, we used deep networks for the \texttaskmodel \space and the differentiable rendering module $\render$, shown in figure \ref{fig:expr_arch}. 

% FIG 3: distribution of costs for toy example [caption revised]

\subsection{Datasets and Benchmark Algorithms} \label{sec:data_schemes}
Recall the dataset notation from Section \ref{sec:proposed_method}.
We compare \texttaskmodels \space trained on the following different datasets:

\begin{enumerate}[leftmargin=*]
    \item \Original: The task model (i.e., both perception and planning models) is \textit{only} trained on the original $\datasetorigtrain$.  
    \item \DataAdded: We add more training examples from the same (or very similar) distribution as the original training dataset, denoted by $\datasetaddtrain$. This tests whether more examples are necessary to achieve better performance. The task model is then trained on the union of the original and added dataset, denoted by $\datasetaddtrain \cup \datasetorigtrain$. 
    \item \DataAug: We apply standard \textit{task-agnostic} data augmentation to the original training data. For the case of image inputs, we applied random contrast, random brightness and random blur to the images $s$. We refer to this widely-used scheme as task-agnostic as it solely aims to improve the perception model without accounting for the MPC task. The augmented dataset is denoted by $\datasetaugtrain$ and we re-train the task model on $\datasetaugtrain \cup \datasetorigtrain$.
    \item \TaskDriven \space (Ours): We use Algorithm 1 to synthesize adversarial dataset $\datasetadvtrain$. Then, we \textit{re-train} the task model on $\datasetadvtrain \cup \datasetorigtrain$. 
\end{enumerate}

\textit{Test Datasets:}
We test all the above training schemes on several independent, held out test datasets. 
First, we report the accuracy on the original dataset's test images $\datasetorigtest$. Next, we report on OoD dataset $\datasetOoDtest$, such as different weather conditions from the training distribution. 
Then, to confirm the rendered scenarios are indeed adversarial, we also report performance on the adversarially perturbed versions of the original test dataset $\datasetadvtest$, which are generated by Alg. 1. 

\subsection{Illustrative Toy Example: 2D Obstacle Avoidance.} 
\label{sec:toy_obs}
We now introduce a simple task  where a planar 2-D robot has to navigate around obstacles to reach a goal location, as pictured in Fig. \ref{fig:toy_adv_scenarios}. This experiment demonstrates how adversarial training creates more challenging scenarios for the \texttaskmodel \space to plan in. 
\SC{Furthermore, we quantitatively show that a \texttaskmodel \space trained on adversarial scenarios $\datasetadvtrain$ learns to avoid collisions more successfully and with lower control cost compared to standard training procedures.} 
\input{figures_latex/toy_scenario_col}
%the \texttaskmodel \space trained on $\datasetorigtrain$ and $\datasetaddtrain$.}

%\textit{Experimental Settings: }
% \input{figures_latex/toy_adv_scenrio}

The input to the 2-D planar robot is a $100\times100$ grey-scale image $s$ of the scene, including obstacles and the goal $g$, indicated by a star-shaped marker. Given the sensory input $s$, the \texttaskmodel \space $\alltaskmodel$ is a perception-planning module that outputs a sequence of future waypoints $w_F$ for the robot to navigate. \SC{A waypoint $w_F$ is simply a pose the robot must move to in the $xy$ plane.}
The \texttaskmodel \space $\mtaskmodel$ uses a history of past waypoints $w_P$ to improve its predictions. 
The linear MPC task cost is defined in Eq. \ref{eq:track_mpc}.
%The linear MPC task cost for trajectory tracking is defined in Eq. \ref{eq:track_mpc}.
%The \texttaskcost \space is a standard quadratic tracking cost with linear obstacle avoidance constraints defined in Equation \ref{eq:track_mpc}.

% \input{figures_latex/collision_table}
% \input{figures_latex/collision_toy_scenario}

We synthetically created the training $\datasetorigtrain$ and the held-out test datasets $\datasetorigtest$ and $\datasetOoDtest$ for the experiments. \SC{As shown in Fig. \ref{fig:toy_adv_scenarios}, each scenario had randomly generated ellipsoid obstacles with random sizes and locations.} 
The ground truth waypoints $y = w_F$ are generated using a standard Frenet Planner \cite{frenet2010werling} that has full access to all obstacles and start/goal locations for the entire scene. The synthetic dataset contained $|\datasetorigtrain| = 7000$ training scenarios and $|\datasetorigtest| = 2200$ test scenarios. A larger similar dataset had $|\datasetaddtrain| = 10000$ training examples. \SC{Another dataset of $|\datasetaugtrain| = 10000$ training examples was generated from task-agnostic data augmentation.} The synthetic adversarial dataset generated by our method had
$|\datasetadvtrain| = 10000$ training scenarios and $|\datasetadvtest| = 2200$ adversarial test scenarios. \SA{We used $K=10$ gradient steps in Algorithm \ref{alg:train} to generate the adversarial scenarios.} Finally, we also generated a challenging OoD test dataset, $\datasetoodtest$, where the ellipsoid obstacles were samples from a different distribution than the original dataset $\datasetorigtrain$. Specifically, ellipsoid obstacles were bigger and closer in the OoD test dataset, thus making it hard for the robot to plan.  We use a history of $P=10$ past waypoints to predict the next $F=20$ future waypoints.


The experiment shows that training the \texttaskmodel \space with additional adversarial data using Alg. 1 leads to superior performance compared to all benchmarks described in Sec. \ref{sec:data_schemes}.
We quantitatively compare the performance of all benchmarks on the number of collisions with obstacles, the average \texttaskcost \space $\taskcost$, and the mean-squared error (MSE) in predicting the waypoints on all test datasets. 
\SC{Finally, we qualitatively show that our rendered scenarios are adversarial and realistic compared to the training distribution}.
% \input{figures_latex/toy_scenario_col}

% FIG3: collision table [caption revised]
\input{figures_latex/combined_metrics}
% \input{figures_latex/toy_metrics}

% \input{figures_latex/xplane_metric}

\textit{Quantitative results: }
\SC{Table \ref{tab:toy_collision}} shows the number of scenarios with collisions for all training schemes. Our \TaskDriven \space approach was able to perform as well as the \DataAug \space, \DataAdded \space, and \Original \space benchmarks on the original test dataset. Additionally, the \TaskDriven \space approach significantly outperformed the \DataAug \space scheme by $49\%$, \DataAdded \space scheme by $67\%$ and \Original \space scheme by $69\%$ on the adversarial test dataset $\datasetadvtest$. Furthermore, our \TaskDriven \space approach outperformed the \DataAug \space scheme by $15.8\%$, \DataAdded \space scheme by $30.8\%$ and \Original \space scheme by $38.6\%$ on the unseen OoD test dataset $\datasetoodtest$. \SC{Thus,}  our training scheme \textsc{Task-Driven} leads to significantly fewer collisions on challenging OoD scenarios.

% caption edited
% Fig 4: qualitative results [caption revised]

\SC{We now illustrate that our scheme also reduces the MPC task cost $J$}.
Fig. \ref{fig:combined_metrics} (top left) shows the MPC task cost for all training schemes on 2200 held-out test datasets. On the original test dataset, our \textsc{Task-Driven} scheme (red) performs on par with the \textsc{Original} (blue) scheme and slightly worse than the \textsc{Data-Added} (orange) and \DataAug \space (green) schemes. The \textsc{Data-Added} scheme's performance is expected because it is trained on more original data than our \textsc{Task-Driven} scheme, which allows it to perform
slightly better on the original test dataset. However, the key benefits of our approach are shown on the synthetic adversarial test dataset and held-out OoD dataset. The key take-away is that our scheme significantly outperforms the \DataAug \space scheme, with $204 \%$ less average MPC cost (Wilcoxon p-value of $0.0$) on the synthetic adversarial test dataset and $80 \%$ less average MPC cost (Wilcoxon p-value of $0.0$) on the held-out OoD dataset.

We now illustrate why our method is able to reduce the ultimate task cost. Specifically, Fig. \ref{fig:combined_metrics} (top right) shows that our \textsc{Task-Driven} scheme achieves lower MSE for predicting ground-truth waypoints from the Frenet Planner than competing benchmarks. While all methods perform similarly on the original test dataset, the key gains of our scheme are on the adversarial test dataset and held-out OoD dataset. Our scheme significantly outperforms standard data augmentation by achieving $264.5 \%$ less average waypoint MSE on the synthetic adversarial test dataset and $4.5 \%$ less average waypoint MSE on the held-out OoD dataset.

\textit{Qualitative Results: }
Fig. \ref{fig:toy_adv_scenarios} shows a challenging adversarial scenario that is automatically synthesized by our method in dataset $\datasetadvtrain$. Our training scheme brings obstacles closer to the robot's originally intended waypoints and path, making it harder to find a collision-free path. Naturally, this increases the \texttaskcost \space since the robot has to make wider turns and swerves. Therefore, rather than augmenting our dataset with well-understood scenarios already reflected in the training distribution, our scheme targetedly adds challenging scenarios that make the model more robust.

\subsection{\SC{X-plane: Autonomous Vision-Based Airplane Taxiing}} 
\label{sec:xplane_epr}
\SC{We now} test our method on an autonomous aircraft taxiing problem. 
\SC{As shown in Fig. \ref{fig:adv_scenarios}, the airplane has a wing-mounted camera and passes the images through a perception model to estimate its distance and heading angle relative to the center-line of a runway. Then, it uses differentiable MPC to navigate to the runway center-line with minimal control cost. We use a public dataset from the photo-realistic X-Plane simulator \cite{XPlane} consisting of images from the plane's wing-mounted camera in diverse weather conditions and at various poses on the runway. This standard
benchmark dataset has been used in recent works on robust and verified perception \cite{taxinetDataset,sharma2021sketching,katz2021verification}. Our prime goal is to test that our adversarial training method yields models that outperform benchmarks at generalizing to challenging OoD weather conditions.}
%compared to standard task-agnostic data augmentation.}

\subsubsection{Setting}

The input to our \SC{``robot''} is a $128\times128$ RGB image $s$ of the runway taken from the right wing. The \texttaskmodel \space $\alltaskmodel$ is a perception-planning module that outputs the desired pose of the airplane $w_F$, given this sensory input $s$ and \SC{a} history \SC{of} waypoints $w_P$. Specifically, the \texttaskmodel \space outputs \SC{a} single waypoint $w_F$, which is a tuple of the distance
to the centerline of runway $c$ and the heading angle $\theta$, denoted by $w_F = {(c_i, \theta_i)}_{i=0}^{F}$ for $F=1$. $w_P = {(c_i, \theta_i)}_{i=0}^{P}$ is a history of \SC{the} $P = 10$ past waypoints which are used to improve the planning model's predictions. MPC with linearized dynamics (Eq. \ref{eq:track_mpc}) is used to plan a sequence of controls to navigate to the center-line.

% It is important to note that in this setting, the \texttaskmodel only outputs the current state of the aeroplane. Tracking vector $\mathbf{w}_F$ for the mpc is a $F$ length vector of tuples $w_F = {(0, 0)}_{i=0}^{F}$, since we want the distance to the centerline and the headling angle to be 0. An example of the task scenario is shown in figure \ref{fig:xplane_scenario}. 

\textit{Images from Diverse Weather Conditions: }
We will represent the whole X-plane dataset as $ \Gamma = \{ \datasetafternoon, \datasetmorning, \datasetovercast, \datasetnight \} $, where each dataset \SC{corresponds to the subscripted} weather condition. Each individual weather dataset in $\Gamma$ has $44,000$ training scenarios and $11,000$ testing scenarios. \SC{Ground truth waypoints are obtained from the X-Plane simulator}. 
%\SC{Ground truth waypoints obtained from the X-Plane simulator} are part of the dataset. 

\SC{Our goal is to establish that we can re-train a perception model that robustly generalizes (with good control performance) to OoD weather conditions. To do so, we start with a perception model that is \textit{initially} only trained on afternoon conditions and evaluate its performance on held-out test images across OoD weather conditions.}
\SC{To do so,} we will compare 4 different task models $\mtaskmodel$. The \textsc{Original} model is only trained on $\datasetafternoontrain$, \SC{while the} \textsc{Data Added} model is trained on $\datasetaddtrain = \datasetafternoontrain \cup \datasetmorningtrain$ since the morning and afternoon are visually similar. 

\SC{Today's standard benchmark of task-agnostic data augmentation} is trained on $\datasetaugtrain = \datasetafternoontrain \cup \datasetaugtrain$, where we perform image augmentations (random crops, rotations, and hue alterations) on the original afternoon training data using the open-source Albumentations library \cite{albumentations}. 
\SC{Finally, our} \textsc{Task Driven} model is trained on $\datasetafternoontrain \cup \datasetadvtrain$, where $\datasetadvtrain$ are adversarial scenarios created using our method applied to the original afternoon training data. \SA{We trained the adversary for $K=15$ steps in Algorithm \ref{alg:train}.} 
We quantitatively compare the performance of all benchmark task models on mean task cost $\taskcost$ and waypoint MSE on held-out test datasets for each condition,
such as afternoon, morning, night (OoD), and synthetic test images ($\datasetadvtest$).


% Figure 5: X-Plane Boxplots [caption revised]
\input{figures_latex/xplane_adv_scenario}
% \input{figures_latex/combined_scenario}


\subsubsection{Quantitative results}
We \SC{now} show that our \textsc{Task-Driven} scheme reduces the average \texttaskcost \space $\taskcost$ compared to other \texttaskmodels. Fig. \ref{fig:combined_metrics} (bottom left) shows the average \texttaskcost \space (Y-axis) for all the \texttaskmodels \space when evaluated on different test data scenarios (\SC{X-axis}). On the \SC{afternoon and morning test scenarios}, our \textsc{Task-Driven} scheme (red) performs on par with other \texttaskmodels. This is expected because all
networks are trained on this data. Since the morning data is \SC{visually similar to the} afternoon data, the \texttaskmodels \space perform similarly as well.
% The \texttaskmodel \textsc{Data Augmentation} is not able to help much since it is only creating single-step data augmentations, i.e. augmentation relevant only for perception \texttaskmodel but not for planning \texttaskmodel.

However, the key benefits of our approach are highlighted in the \SC{OoD} \SC{night and synthetic adversarial test datasets}. %$\datasetnighttest$ and $\datasetadvtest$. 
Our method automatically generates examples of challenging scenarios from the original afternoon training dataset and adds them to $\datasetadvtrain$, making the \textsc{Task-Driven} \texttaskmodel \space robust to \SC{OoD} test datapoints as shown in the night and synthetic adversarial columns in Fig. \ref{fig:combined_metrics}. The \textsc{Data Augmentation} \texttaskmodel \space cannot help that much since it only creates single-step data
augmentations that are often relevant only for the perception model but not necessarily for planning or control. Our \textsc{Task-Driven} scheme has $28.2\%$ less average cost (Wilcoxon p-value of $0.0$) for the night test dataset and $16.6\%$ less average cost (Wilcoxon p-value of $0.0$) for the synthetic adversarial test dataset compared to standard data augmentation. 

Figure \ref{fig:combined_metrics} (bottom right) shows how our \textsc{Task-Driven} scheme achieves lower MPC task cost by predicting future waypoints $w_F$ with lower MSE. While all methods perform similarly on the original test dataset $\datasetafternoontest$, the key gains of our scheme are on the night and synthetic adversarial test datasets. %$\datasetnighttest$ and $\datasetadvtest$. 
Specifically, the \textsc{Task-Driven} scheme has $54.7\%$ less average cost (Wilcoxon p-value of $0.0$) for the night test dataset and $42.6\%$ less average cost (Wilcoxon p-value of $0.0$) for the synthetic adversarial test dataset compared to standard data augmentation. 


\textit{Qualitative Results: } 
We now provide intuition for how our \textsc{Task-Driven} scheme outperforms standard benchmarks by illustrating challenging adversarial scenarios that we automatically synthesize in dataset $\datasetadvtrain$. \SC{Fig.} \ref{fig:adv_scenarios} shows two scenarios where our adversarial training scheme \SC{makes it harder} to detect the runway center-line. On the left of Fig. \ref{fig:adv_scenarios}, the weather condition stays the same,
but the centerline is blurred like in a foggy condition. On the right of Fig. \ref{fig:adv_scenarios}, adversarial training changes the afternoon weather condition to night, which the \textsc{Original} \texttaskmodel \space has never seen before. Naturally, this increases the \texttaskcost \space since the original task model mis-estimates the faintly visible center-line on the top left. As such, our scheme targetedly adds challenging scenarios to make
the task model more robust. 

%%% describe VAE training caveat

It is important to note that the original renderer was trained on night training images so that the VAE can render a night scene in the first place. However, we strictly only trained the initial perception and planning models on the original afternoon training data. As such, they were never exposed to a single night (OoD) image. This scenario is practically motivated as, in reality, differentiable renderers have the ability to map a continuum of scene parameters
$\nu$ to scenes $s$, but
we can only train the task model on a finite set of scenes $\nu$ from a specific training distribution for cost-effective training. As such, our result illustrates that adversarial scenario generation can efficiently find and render scene parameters $\nu$ that were not seen in the task model's original training distribution. Naturally, for a fair comparison, all benchmarks used the same VAE renderer that was pre-trained initially and had frozen weights during adversarial scenario generation.

% \input{figures_latex/combined_xplane_adv_tsne}

Finally, Fig. \ref{fig:xplane_latent} shows the relative distance between different test datasets' latent variables when projected in a 2D space using the t-SNE method \cite{hinton2002stoc}. 
Interestingly, our task-driven scheme is able to add synthetic data points (yellow) that emulate, and anticipate, the OoD night distribution. However, points added by standard data augmentation (pink) do not overlap much with the night data (green), explaining why the benchmark generalizes more poorly. 
%This figure showcases why our training scheme \TaskDriven \space can generalize to OoD data while other training schemes cannot.

\textit{Limitations: } In future work, we aim to develop theoretical generalization guarantees, at least for a linear adversary, simple generative model, and linear MPC.

\input{figures_latex/latent_xplane}
%Moreover, we need automatic methods to set consistency loss weight $\kappa$.
%Rather than augmenting our dataset with well-understood scenarios already reflected in the training distribution, our scheme targetedly adds challenging scenarios that make the \textsc{Task-Driven} \texttaskmodel \space more robust. 



==> sections/somi_edits/experiment_procedure_backup.tex <==
\textit{Experiment Procedure: } In all three domains, we first trained a VAE on all the dataset. Next, we trained the task model (perception and planning models) for a subset of training data as defined in Sec. \ref{sec:data_schemes}. The \texttaskmodel \space $\alltaskmodel$ is a perception-planning module that maps a sensory input $s$ and waypoint history $w_P$ to a sequence of future waypoints $w_F$ for the robot to navigate towards. The MPC task cost is defined in Eq. \ref{eq:track_mpc} and further implementation details are described in Appendix \ref{sec:appendix_experiment_details}. We now evaluate the performance of all the different training schemes on OoD test datasets.

% \subsection{Experiment Procedure} \label{sec:expr_proc} 
In the simple 2-D planning task a robot has to navigate around obstacles (large ellipsoids) to reach a goal location (green star) as shown on left in Fig. \ref{fig:combined_qual_images}. In the Robosuite manipulation task, a \textit{Franka} arm needs to pick a blue ball while avoiding red boxes as shown in center in Fig. \ref{fig:combined_qual_images}. In the manipulation task we only control the arm in task-space using MPC and use built-in controllers in Robosuite to control \textit{Franka} \cite{frankaemika} arm joints. Finally in the the X-plane experiment the airplane has a wing-mounted camera and passes the images through a perception model to estimate its distance and heading angle relative to the center-line of a runway. Then, it uses differentiable MPC to navigate to the runway center-line with minimal control cost. We use a public dataset from the photo-realistic X-Plane simulator \cite{XPlane} consisting of images from the plane's camera in diverse weather conditions and at various poses on the runway. This standard
benchmark dataset has been used in recent works on robust and verified perception \cite{taxinetDataset,sharma2021sketching,katz2021verification}.

